TelApart: Differentiating Network Faults from Customer-Premise Faults in Cable Broadband Networks

Two types of radio frequency (RF) impairments frequently occur in a cable broadband network: impairments that occur inside a cable network and impairments occur at the edge of the broadband network, i.e., in a subscriber's premise. Differentiating these two types of faults is important, as different faults require different types of technical personnel to repair them. Presently, the cable industry lacks publicly available tools to automatically diagnose the type of fault. In this work, we present TelApart, a fault diagnosis system for cable broadband networks. TelApart uses telemetry data collected by the Proactive Network Maintenance (PNM) infrastructure in cable networks to effectively differentiate the type of fault. Integral to TelApart's design is an unsupervised machine learning model that groups cable devices sharing similar anomalous patterns together. We use metrics derived from an ISP's customer trouble tickets to programmatically tune the model's hyper-parameters so that an ISP can deploy TelApart in various conditions without hand-tuning its hyper-parameters. We also address the data challenge that the telemetry data collected by the PNM system contain numerous missing, duplicated, and unaligned data points. Using real-world data contributed by a cable ISP, we show that TelApart can effectively identify different types of faults.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=paper

PDF = $(PACKAGE).pdf
SRCs = $(wildcard *.tex)

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF}

#%.pdf:  %.dtx   $(PACKAGE).cls
%.pdf:  %.tex ${SRCs}
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> align.tex <==
\subsection{Align Data Points}\jy{Ready to read}\label{sec:align}\jy{not interesting}

%After obtaining all the positions of missing data for each modem, we then divide the missing into 3 different types: Channel Missing, Partial Missing, and All Missing. Since we collected the PNM data from 3 upstream channels at the same time, it is possible that we can only collect the data from 1 or 2 channels, but fail on the others. All Missing and Group Missing are distinguished by other modems using the same \FN. If we observe that all the modems in the same \FN have missing data points at the same time, \zzy{How do you define "the same time" without alignment?} we define this type of missing as all missing, otherwise as partial missing. Our assumption is that these two types of the missing will indicate network faults with different granularity.

After inferring missing data points for each device, we aim to utilize clustering algorithms to group the devices with the same abnormal pattern. The first step is to calculate the similarity between the two devices. However, due to network delay and sequential measurement requests caused by low network capacity, the \pnmdata of different devices are unaligned in the time axis. Unaligned data can cause different lengths of time series data \zzy{Although I understand this is because without alignment, there could be multiple data points for 1 CM within a data collection period, this is not quite obvious, because when introducing the reason for alignment, it's mostly time skew, and why there could be more points is not explained. Note that this is also different from missing, where we can have fewer data points, not more.} from different devices and lead to inaccurate \zzy{why is it only inaccurate rather than not possible to compute?} distance measures between the time series, which makes it difficult to calculate the similarity between devices. And the missing data further enhance this difficulty. Therefore, in this section,  we develop an algorithm to align the time series data between pairwise devices so that we can compare the similarity using the same length of time series data between any two devices.

Figure~\ref{fig:align_a} shows an example. Each data point is represented by a small circle and the red circle indicates an inferred missing data point. During the time period $[t_1, t_2]$, device $x$ has 9 data points, and device $y$ has 8 data points. To compare the similarity between the two devices' data, we must establish a one-to-one mapping between these data points. 

We design an alignment algorithm to establish a one-to-one correspondence between two devices' telemetry data after we fill in their missing data points. The goal of this alignment algorithm is to pair up two devices' data points that are collected at the closest time points. The algorithm takes as input two devices' data collection timestamp vectors $T_x = \{x1, x2, x3, x4, x5, x6, x7, x8, x9\}$ and $T_y = \{y1, y2, y3, y4, y5, y6, y7, y8\}$. It first establishes an injection from $T_x$ to $T_y$, by mapping each timestamp in $T_x$ to its closest timestamp in $T_y$, as shown by the blue arrowed lines in Figure~\ref{fig:align_b}. In this step, multiple data points in $T_x$ may map to the same data point in $T_y$. Therefore, we perform the same injection in the reverse direction from $T_y$ to $T_x$, as shown by the dashed orange lines in Figure~\ref{fig:align_c}. Finally, it prunes the pairs where there only exists a one-direction mapping \zzy{bijection?} (Figure~\ref{fig:align_d}).  Now the remaining timestamps in each of the input vectors $T_x$ and $T_y$ have one-to-one correspondence. The algorithm can further prune the pairs where one of the timestamps has a missing data point (Figure~\ref{fig:align_e}). After this step, we generate $T_{x_y} = \{x1, x4, x7, x9\}$ and $T_{y_x} = \{y1, y4, y7, y8\}$. $T_{x_y}$ and $T_{x_y}$ have the same length, so that \sys can compare the similarity between device $x$ and device $y$ using the \pnmdata which are collected from timestamp $T_{x_y}$ and $T_{x_y}$. We include the pseudo-code for this algorithm in Appendix~\ref{appendix:align} as well as a formal proof demonstrating that our alignment algorithm achieves the smallest time difference among all possible alignment results. Therefore, with high probability, it can align the points  collected in the same collection period.
% \xy{Fix the notations in appendix to
% be consistent with the graphs.} \zzy{Done}

We use Figure~\ref{fig:align_d} to explain why we infer missing data
points before we align two devices' data points. The bi-directional
injection approach can pair up the data points in two vectors with
different lengths even without the missing data inference step, as
shown in Figure~\ref{fig:align_f}. However, without inferring the
missing data placeholders, the alignment between two timestamps can easily
cross two different data collection periods, increasing the time
differences between two comparable data points. For example, $x_3$ is
paired up with $y_2$ in Figure~\ref{fig:align_f}, while it should be
ignored as device $y$ misses a data point in the same collection
period. Misalignment reduces the quality of similarity comparison as
the data points being compared are not collected as close in time as
those aligned after we insert missing data points. % We show this algorithm
% in Appendix~\ref{appendix:align} as well as the proof of correctness.

 %and one of the data point is a missing one and each timestamp has a
 %non-missing data point. Therefore, \sys's similiarity comparion
 %function is able to compute a similarity score between the two devices
 %$x$ and $y$.
 %

% 
% 
% The alignment algorithm we design works between each pair of devices:
% $x$ and $y$. We first establish an inject 
% 
% in order to monitor the status
% among multiple devices, we need to compare the metrics collected at a
% similar time. Since only when we calculate the similarity between two
% time series data will we utilize the aligned time between two devices,
% we will focus on the pairwise alignment in this work, which means
% aligning two time series data at a time.
% % We utilize the Algorithm~\ref{alg:align} to align the time series data from different devices. 
% 
% 
% Assume we have two devices $a$ and $b$, their timestamp arrays are $T_a$ and $T_b$ respectively. We first generate an injection $S_{(a, b)}$ \zzy{$a$ is not defined here (I'm aware of its definition in the algorithm). It might be better to make the text self-contained. Also, we can add the line number of the algorithm here, eg. we calculate $S_{(a, b)}$ at Line 3. (This can be a TODO after the algorithm is fixed, no need to do it now if the algorithm is subject to change.)}\jy{Explained. Agree for the line number} from each timestamp in device $a$'s time series data and its closet timestamp in device $b$'s time series data. Then, use the same method to generate an injection $S_{(b, a)}$ from the time series data of device $b$ and device $a$. Then, we put all the pair of $t_{ai}$ and $t_{bj}$ that in both $S_{(a, b)}$ and $S_{(b, a)}$ to $A_{(a, b)}$. Since both $S_{(a, b)}$ and $S_{(b, a)}$ are injections and $A_{(a, b)}$ is a surjection, $A_{(a, b)}$ is a bijection. Each element $(t_{ai}, t_{bj})$ in  $A_{(a, b)}$ means timestamp $t_{ai}$ in device $a$ are aligned with timestamp $t_{bj}$ in device $b$.
% 
% After aligning the time series data for every device pair, we can use the $A_{(a, b)}$ to calculate the distance between the device $a$ and device $b$. For each metric, we can obtain $V_a = \{\textrm{value of this metric for device} \ a \ \textrm{at} \ t_{ai} \ | \ (t_{ai}, t_{bj}) \in A_{(a, b)}$, $t_{ai} \neq \textrm{missing}, \ t_{bj} \neq \textrm{missing}\}$ % \zzy{I guess you're looking for $\backslash textrm$?}\jy{Do not understand here} 
% from device $a$ and $V_b$ from device $b$. Then, $V_a$ and $V_b$ are two vectors with the same length. Therefore, we can use the common similarity/distance metrics to calculate the similarity between device $a$ and device $b$. However, the length of $V_a$ is variable, since it depends on how many data points from device $a$ and device $b$ are missing. If the length of $V_a$ and $V_b$ are too small, \zzy{This is a little misleading, what if $V_b$ is too short? Then the reader needs to figure out the two vectors have the same len and this actually also implies the case for short $V_b$.}\jy{Fixed} we will label these two devices as incomparable, since we wants enough evidence to present the metrics patterns of these two devices are the same. 
% 


==> cut-off.tex <==
\if 0
The first challenge we encountered for evaluating \sys is the lack of ground truth. Unlike supervised solution that can be easily validated by labels, it is infeasible for us to know exactly when a maintenance issue starts and ends, as well as which users are affected.
This is a natural result of the lack of a tool diagnosing maintenance issues.
% the fact that nowadays ISPs still heavily rely on manual efforts to detect maintenance issues.
% ISPs record historical issues (\eg, by labelling tickets) according to their operating experience but such labelling needs significant human intervention and is error-prone.

In order to evaluate how accurately \sys can distinguish maintenance issues, we manually labeled a small fraction of our data to obtain the ground truth. For use the maintenance tickets as hints to help us label the data based on an assumption: if there is a maintenance ticket that happened at time t, it has a higher chance for us to observe abnormal patterns from our telemetry data during that time. Therefore, for each maintenance ticket that we received from a device, we manually check all the performance metrics from our telemetry data that were collected between t - 1 week and t. If we observe more than 5 devices have the same abnormal pattern on either of the performance metric, we will record all the devices that have this pattern as a cluster that is affected by a maintenance issue. For the cluster whose size is less than 5, we will label this issue as a service issue. It is possible that we can observe more than 1 maintenance issue around maintenance tickets, or cannot observe any abnormal patterns since the network issue cannot be detected by our telemetry data. We have checked more than 50 maintenance tickets, and only 13 of them help us find maintenance issues that can be detected by our data. Our labeling contains 16 groups of maintenance issues 
together with 113 devices that were affected by service issues, and carefully verified the labeling results with \anonisp's experts. Such manual labeling efforts are not scalable and we intentionally maintain a relatively small dataset to guarantee the labeling accuracy. Table~\ref{tab:manual_label_result} shows the results that we applied representative clustering algorithms including \sys's onto this manually labeled dataset.
\fi

\if 0
Manually labeling data costs a great number of human resources, which prevents us from evaluating the performance of \sys on a large scale. In order to analyze the performance of \sys over all the datasets we have, we use customer-reported tickets as hints to help us evaluate the performance of \sys. In our data, we call primary tickets and part of primary tickets \emph{maintenance tickets} and the other tickets \emph{service tickets}. These two types of tickets can help us evaluate the performance of \sys: if the maintenance issues our clustering algorithms detected are highly correlated with the maintenance tickets, the effectiveness of \sys is demonstrated. 

However, we cannot use the maintenance tickets as the ground truth since they have much noise. A maintenance team may label service tickets as maintenance tickets since the two issues happened at the same time. Several tickets that complain about the same maintenance issue may be attached to 2 primary tickets since the maintenance team thinks those tickets complain about different issues. In order to mitigate the noise, we borrow the idea from~\cite{hu2020cablemon} to quantify the correlation between maintenance issues and maintenance tickets. In this work, the authors define \emph{ticketing rate}, which indicates the number of tickets observed in a unit of time. Similarly, we define \emph{maintenance ticketing rate} using maintenance tickets only. In order to calculate these two metrics, we first implement the algorithm presented in~\cite{hu2020cablemon} to obtain abnormal events by TX power, SNR, and missing. Our implementation is confirmed by the authors. Each abnormal event represents a network issue that observed on a single device by one of those diagnosis metrics during a time period, from $t_l$ to $t_r$. For each abnormal event, our clustering algorithm checks whether other devices in the same fiber optic node have the same abnormal pattern. If there are less than 5 devices in the cluster, we will label it as a service issue, otherwise a maintenance issue. This threshold is recommended by our cooperating ISP. If there are $n$ devices in this cluster, and those devices report $x$ maintenance tickets between $t_l$ and $t_r$, we can calculate the maintenance ticketing rate by $r = x/((t_l-t_r)*n)$. We can calculate the overall maintenance ticketing rate by summing over all abnormal events as $r_{all} = \frac{\sum_i x_i}{\sum_i (t_{l_i} - t_{r_i}) * n_i}$.

Given the concept of maintenance ticketing rate, we can tune the parameters of \sys and compare it with other algorithms. \sys only requires one threshold: when we build a graph, if the similarity between two devices is larger than the threshold, we will add an edge between these two devices. We select the value which can give us the best maintenance ticketing rate, and compare the maintenance ticketing rate with other clustering algorithms. Besides, we also manually labeled several maintenance issues and services issues, in order to compare the performance of \sys and other clustering algorithms using external criteria.
\fi

\if 0
Manually labeling data costs a great number of human efforts, which
prevents us from evaluating the performance of \sys on a large
scale. In order to analyze the performance of \sys over all the
datasets we have, we use the normalized ticketing rate introduced in
~\S~\ref{sec:eval_method}. Since \sys is invoked by a triggering
device that suffers a network anomaly event $e$, we adopt
CableMon~\cite{hu2020cablemon} on our data for the entire data
collection period to obtain the anomaly events that can be detected by
SNR, Tx power, and missing. We then run \sys and other clustering
algorithms on each triggering event, then calculate the overall
normalized ticketing rate for each metric, as well as the combined
normalized ticketing rate for all metrics.
\fi

% Let $m$ to denote maintanence and $s$ to denote service. First,


==> deploy.tex <==
\subsection{How to Deploy \sys}
\label{sec:deploy}

% Include a table of all hyper-parameters \sys uses, their
% definitions, and how to set their values.

Any cable ISP that collects \pnmdata can deploy \sys to improve cost
efficiency in the following steps.

First, an ISP will run \sys's training module to determine its
hyper-parameters using its historic PNM and customer-ticket data
collected from its networks. An ISP can conduct this step
periodically to cope with model drift.

% We note that an ISP need not hand-tune any hyperparamter.

After the training step, an ISP can deploy \sys in either a \proactive
or a \reactive. In the \proactive, an ISP periodically invokes \sys to
monitor its networks (\eg, every data collection interval). Based on
\sys's diagnoses, it can proactively repair maintenance or service
issues before customers react to them. In the \reactive, an ISP
invokes \sys when it receives a customer call and employs \sys's
diagnosis to make a dispatch decision.

% \zzy{Shall we change all "online mode" back to "reactive mode"? Now this is inconsistent from other sections.}

% If we find the collection
% time interval of two adjacent \pnmdata points exceeds
% $thr_{missing}$ hours, we consider there are missing points between
% those two adjacent points. To find the best value of
% $thr_{missing}$, we compare the missing point inference accuracy
% against the ground truth generated by clustering on historical data
% for a $thr_{missing}$ value, and pick the one with the highest
% accuracy, as described


==> design-old.tex <==
\if 0
\section{Design Overview}\label{sec:design}


\subsection{Goals}

We assume that there exists an anomaly detection method that signals
anomalous devices to a cable ISP (\S~\ref{sec:anomaly}). So the main
goal of this work is to automatically differentiate the types of
faults, \ie, a maintenance issue or a service issue, that lead to
anomalies. Detailed diagnosis of a faulty component involves
measurements of the physical network infrastructure. Hence, it is
beyond the scope of this work. We aim to accurately diagnose the type
of a fault so that an ISP can dispatch the correct technical personnel
to the appropriate location for a more detailed component-level
diagnosis. More specifically, we aim to be both effective and
efficient in \sys's design. We describe each goal in turn. 

\begin{itemize} [topsep=0.1ex,leftmargin=2\labelsep,wide=0pt]
        \setlength\itemsep{0em}
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\item \textbf{Effective:} \sys should accurately diagnose the type of
  a fault that causes an anomaly. That is, when an anomaly is caused
  by a maintenance issue (or a service issue), \sys should identity it
  as a maintenance issue (or a service issue) with high probability.
\end{itemize}

\fi

% solution: we first infer the missing data and then invited an alignment algorithm. We do not require all the modems have the same length of vectors. Instead, we require pair-wise similarity measurement. 

% \begin{figure}[tb!]
% \centering
%     \includegraphics[width=.45\textwidth]{./figures/align1.eps}
%     \label{f:align1}
% \end{figure}

% challenging2: which similarity metric should be used?
% solution: txpower/snr/rxpower: Pearson similarity; uncorrectable/missing: Normalized Hamming distance
% 
% challenging3: cannot compare the similarity between some pair-wise modems
% solution: interpolation does not work well, since anomaly is unpredictable. Hierarchical clustering may fail if we assign the incomparable pair-wises modems a very large distance or very small distance. Show examples for single-linkage, complete-linkage, and average linkage.
% To overcome this, we use a community detection algorithm
% 
% challenging4: cannot evaluate it. we use both manually labeling and ticket
% solution: tickets
% 
% why this community detection based algorithm works: ~\cite{ferreira2016time}
% 

\section{Design} 

Before describing \sys's design details, we present an overview. We have an assumption here that an ISP has a single-device diagnosis tool such as CableMon~\cite{hu2020cablemon} to identify whether a single device suffers from a hardware-related anomaly. \sys treats the telemetry data collected from each device as time-series data. It takes the time-series data in a time period from all devices served by the same fiber optic node as input, and outputs clustering groups. Devices in the same group share the same \pnmdata pattern. If a device is detected as an anomaly by the single-device diagnosis tool, the entire group will be labeled as an abnormal group, which indicates this group is suffering from a network outage. ISPs can determine whether there is a service issue or maintenance issue by checking the size of an abnormal group. In this work, we set this threshold to be 5 based on the suggestions from \anonisp. If an abnormal group contains fewer than 5 devices, \sys reports a service issue, otherwise a maintenance issue.
 
\sys can operate in two modes: reactive and proactive mode. In a reactive mode, a network operator invokes \sys when an event such as a trouble ticket occurs and the network's single-device diagnosis tool signals that there is a hardware-related anomaly. In a proactive mode, \sys is invoked periodically, \eg, at 5 AM every day. For each fiber optic node, \sys will output several clusters of modems. The network operator scans every device in each cluster. If they detect an anomaly on one device, the operator will label the entire cluster as abnormal. Then the network operator uses the size of the cluster to diagnose whether it is a maintenance or service issue. 

Suppose \sys runs at time $t$, which is either triggered by a trouble ticket or invoked proactively. \sys takes the telemetry data collected in the previous $d$-day period: $[t-d,  t]$ from each device in the same fiber node as the input. The look-back time $d$ is a configuration parameter. In this work, we follow \anonisp's suggestion, set $d = 1$ day. To overcome the first and second challenges described in \S~\ref{sec:challenges}, for each such device, \sys first infers the missing telemetry data points for that device if there is any (\S~\ref{sec:infer}). Then for each pair of devices in the same fiber node, it aligns their telemetry data points (\S~\ref{sec:align}) so that we can calculate the similarity between the two devices. In the meantime, for each telemetry metric useful for network fault diagnosis, it computes a corresponding similarity score between the two devices for that metric (\S~\ref{sec:feature}). Finally, it uses an average linkage hierarchical clustering algorithm to cluster devices with similar anomaly patterns together (\S~\ref{sec:clustering}). We also show how we use customer tickets to help us find the best parameter for the clustering algorithm in this section, which overcomes the third challenge. 






\input{feature}


% \input{similiarity}

\input{clustering}

%\input{parameters}


==> efficiency.tex <==
\subsection{Efficiency}
\label{sec:efficiency}
One design goal of \sys is to be computationally efficient so that an
ISP can run it on a single commodity VM. In this subsection, we
analyze its computational complexity and estimate its computational costs.

% will first discuss the time complexity of \sys, and then show the
% estimated cost when we run \sys using public VMs.

\paragraph{Computational Complexity Analysis} It takes four
computational steps for \sys to partition devices within the same \FN
into distinct clusters with different anomaly types: 1) infer missing
data for each device; 2) align pair-wise devices' telemetry data; 3)
calculating pair-wise similarity scores; and 4) clustering. For each step, the 
time complexity is described in Appendix. Suppose the
input data length is $L$, and the total number of devices in an \FN is
$M$. The computational complexity of \sys is $O(M^2\times L)$.

\paragraph{Estimated Computational Costs} We aim to estimate the
monetary costs for supporting \sys's computation in a public cloud, as
it is the desired deployment mode of \anonisp. We use a server with
one Intel E5640 Xeon processor core and 1 GiB memory to emulate an
Azure Standard\_B1s general purpose VM\cite{microsoft2022bseries} % \jy{cite this: https://docs.microsoft.com/en-us/azure/virtual-machines/sizes-b-series-burstable}. 
We find that for our
dataset, it takes about 30 minutes for \sys to complete the daily
computation when the number of lookback days is set to seven. The
daily input data file size is less than 100M bytes. By the time of
this writing, an ISP can rent an Azure B1s general VM to finish this
computation, which costs less than eight dollars per month.

\paragraph{Time Complexity Analysis} It will take 5 steps for \sys to convert the input data to the clustering results. For each fiber optic node, let us assume there are $n$ cable devices, and each device contains $k$ data points for each channel. Then, we will use this setting to analyze the time complexity for each step respectively. 
\begin{enumerate}[topsep=0pt]
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \item \textbf{Infer Missing Data.} For each device, \sys will iterate each data point once. So the complexity is $O(nk)$
    \item \textbf{Align Time Series Data.} This algorithm will obtain the pairwise alignment for all devices. For each alignment, it will iterate each device's time series data twice. So the complexity of this step is $O(n^2k)$.
    \item \textbf{Calculating Pairwise Similarity.} \sys requires pairwise Pearson correlation coefficient, which will have a complexity of $O(n^2k)$ as well.
    \item \textbf{Cluster Devices.} When build the graph, we need to check all the pairwise similarity, which will cost $O(n^2)$. And Louvain algorithm has a $O(nlogn)$ complexity~\cite{lancichinetti2009community}. 
    %\item \textbf{Detecting Abnormal Clusters.} We adopt CableMon~\cite{hu2020cablemon} to check whether each cluster shows anomalies. The time complexity of this step is $O(nk)$.
\end{enumerate}

Therefore, the complexity of the entire process is $O(nk)$ + $O(n^2k)$ + $O(n^2k)$ + $O(n^2)$ + $O(nlogn)$ = $O(n^2k)$

\paragraph{Estimate Cost on VM} We also deployed \sys on a public VM to estimate the cost when we aim to run \sys daily. We select 1-week data from our dataset from 12/25/2019 to 12/31/2019. It includes more than 60,000 modems from 357 \FNs. The input file size is less than 100M Bytes. Due to NDA, we did not put our data in any public cloud. Instead, we ran \sys in our own machine with recourse limitation. We run \sys with one Intel E5640 Xeon processor core and 1 GiB memory. \sys takes nearly 30 minutes to finish all the tasks. If we use Azure B1s
general purpose VM, it will cost \$7.59 per month.


==> infer-missing.tex <==
\subsubsection{Inferring Missing Data Points}
\label{sec:infer}

\begin{figure}[b!]
\centering
    \includegraphics[width=.40\textwidth]{./figures/interval.eps}
    \caption{\small\textbf{This figure shows the probability density function of data collection intervals.}}
    \label{f:missing_interval}
\end{figure}

\begin{figure*}[th!]
\centering \subfigure[]{
  \includegraphics[width=.32\textwidth]{./figures/align2.eps}
    \label{fig:align_a}
    }
    \subfigure[]{
    \includegraphics[width=.32\textwidth]{./figures/align3.eps}
    \label{fig:align_b}
    }
    \subfigure[]{
    \includegraphics[width=.32\textwidth]{./figures/align4.eps}
    \label{fig:align_c}
    }
    \subfigure[]{
    \includegraphics[width=.32\textwidth]{./figures/align5.eps}
    \label{fig:align_d}
    }
    \subfigure[]{
    \includegraphics[width=.32\textwidth]{./figures/align6.eps}
    \label{fig:align_e}
    }
    \subfigure[]{
    \includegraphics[width=.32\textwidth]{./figures/align7.eps}
    \label{fig:align_f}
    }
    \caption{{\small{\bf This figure shows the steps in \sys's data alignment algorithm.}}\label{fig:align}}
\end{figure*}

% \begin{figure}[tb!]
% \centering
%     \includegraphics[width=.45\textwidth]{./example_figures/design_rationale2.png}
%     \caption{\label{f:design_rationale2}}
% \end{figure}


A monitoring server collects \pnmdata from each device periodically
and unreliably. A data collection request may not receive a response due to packet loss, timeout, or destination unreachable. We call it a missing data point. Missing data points are valuable since they can indicate both availability and reliability issues. Missing data points caused by packet loss and timeout reflect the unreliable of the cable broadband network, while the missing caused by destination unreachable hints the customers cannot connect to the Internet. However, due to the limitation of the data collection framework, it will not record such missing events. Therefore, whether the collected data contain missing data points is unknown to us.

To address this challenge, we developed an algorithm to infer the missing data points in our data. We highlight two observations. First, most of the data collection intervals are centered around the collection period: four hours. Figure~\ref{f:missing_interval} shows the probability density function of the collection time interval between two data points for each CM. If the collection intervals exceed four hours by a large margin, we can infer one or more missing data points. The second observation is that the data from CMs served by the same \FN will be collected during a short period, ranging from 20 minutes to 2 hours. Data collection times from other CMs can help us verify the correctness of the results of an inferring missing algorithm.

Based on the second observation, we design \sys's missing data inference algorithm as follows. For each device, if there are
two adjacent \pnmdata points whose collection time interval exceeds
$thr$ hours, we consider there is a missing data point, and insert a
placeholder ``missing data point'' into the device's \pnmdata
series. We set the timestamp of this missing data point as four hours
after the previous data point's collection time in the originally
adjacent data points. We show this algorithm in
Appendix~\ref{appendix:infer_missing}.

To find the best $thr$, we generated the ground truth of missing data points based on the third observation. We used a clustering algorithm to cluster the data collection time of all CMs served by the same \FN. Each cluster in the cluster results represents a data collection period. If at period $p_1$, the data of modems $m_1$ and $m_2$ are observed, while at $p_2$, $m_1$ and $m_3$'s data are collected, then at $p_1$, $m_3$'s data is missing. The data of $m_2$ is missing at $p_2$. With this approach, we generated the ground truth of missing data points. 

For a certain $thr$ value, we can obtain the results of inferred missing data points. We compared the inferred results with ground truth using the following approach. Given the data collection time of two adjacency points $t_1$ and $t_2$, if there is a missing data point between $t_1$ and $t_2$, and our algorithm result under the select $thr$ outputs this missing data point as well, then we count it as true positive ($TP$). If our algorithm did not report a missing data point during $t_1$ and $t_2$, we count it as a false negative ($FN$). True negative ($TN$) and false positive ($FP$) are defined in the opposite situation. Then we can calculate the accuracy of the selected $thr$ as $\frac{TN+TP}{TN+TP+FN+FP}$.
% (TN+TP)/(TN+TP+FN+FP). 
We select the $thr$ which gives us the highest accuracy as the threshold used in our inferring missing algorithm. The best $thr$ is 6.51, which achieves 98.73\% accuracy.


==> intro-old.tex <==
% The importance of cable network 
Entering the information age, the demands of broadband access networks have sky-rocket. We rely on broadband access networks for numerous daily activities such as e-commerce, entertainment. Moreover, especially during the current pandemic time, broadband access networks offer us the possibility to work and study remotely. In the US, cable networks are one of the few available infrastructures that can provide broadband Internet access to US homes, and in practice, they also dominate over other alternatives~\cite{}. In many rural areas, cable networks are often the only choice for broadband Internet access.

\TODO{Replace old data}
Surprisingly, given the important role that cable networks are playing in our daily life and the fact that they are already developed for decades of years, poor reliability is still an outstanding problem. This is partly caused by the long development history, which not only leaves the fake impression that the networks are mature enough, but also introduces aged devices. Such old devices, such as connectors and amplifiers, contribute to the low average availability as at most two nines (99\%)~\cite{}, much less than the minimum requirement, four nines 99.99\%, proposed by the Federal Communications Commission (FCC) for the public switched telephone network (PSTN).

% Question to solve: detect the service issue and maintenance issue is important, if maintenance issue, then we may find the the potential locations
Cable ISPs leverage a diagnostic platform called Proactive Network Management (PNM) to troubleshoot their cable networks. PNM helps the ISPs to collect various statistic metrics (called PNM data) from their cable modems to pinpoint potential problems. In this work, we collaborate with a regional cable ISP in the U.S. to understand the cutting-edge techniques the ISP is using and the status quo of their troubleshooting strategies. We refer to this ISP as \emph{\anonisp} for the rest of this paper. We learned from \anonisp that ISPs usually have an internal tool to visualize PNM data on the map, then the ISP's experts need to manually find potential problems from the map before dispatching and confirming. 
% Such approach in practice is ineffective and error prone.

% Question to solve and State-of-Art method
There is only a little work in the literature directly attacking this reliability problem of cable networks. ~\cite{hu2020cablemon} introduces an automatic way to find outages by determining thresholds for selected PNM metrics. Although the proposed algorithm alleviates ISP's manual troubleshooting efforts by pointing out problematic modems, in practice, outages can occur at any location of the network, including devices far away from end-users, which could affect a group of users.
Unfortunately, per-metric thresholds are unable to reveal correlations among PNM data from multiple cable modems. Following the convention of \anonisp, we call the outages only affecting a single user as \emph{service} issues, and the outages affecting multiple users as \emph{maintenance} issues.
Failing to detect maintenance issues could significantly increase the number of reported outages without grouping them by root causes, which in turn increases the number of dispatches. More importantly, dispatching to an end user's home generally cannot resolve a maintenance issue simply because the problematic devices are not located correctly.
As mentioned above, ISPs still need to rely on experts to eyeball the visualized map to find maintenance issues with rules of thumb such as the geographical location of problematic modems. Such manual approach is both ineffective and inefficient. It is tricky, if not impossible, to distinguish outages occurring at similar time period and similar locations, but caused by multiple root causes. Moreover, the experts cannot estimate the impact of the anomaly precisely only according to the map because the map only shows the metric in one time point. Unlike time series data, the instantaneous can be noisy and cannot reveal the trend. 

% Our method
In this paper, we propose \name, a framework that employs unsupervised learning to cluster outages and detect maintenance issues. After pinpointing individual problematic cable modems like status quo, \name clusters cable modems with the same abnormal ``patterns'', which essentially implies the features extracted from each modem's PNM data when the data is treated as time series. \TODO{Jiyao: can you add a figure here to explain "patterns"?} \name is able to help ISPs distinguish service issues and maintenance issues, more accurately locate the root cause, and as a result, save dispatches and operating cost, as well as improve customer experience.

We are facing the following challenges when designing \name: (1) Classic clustering algorithms like DBSCAN~\cite{} cannot be applied to PNM data directly. This is because PNM data is collected with UDP, an unreliable transport protocol. Hence, data point occurrence (e.g., caused by lost response) cannot be guaranteed. With such missing data points, it is infeasible to define the pairwise distance between PNM data of two modems because the collection timestamp of their non-missing data points may not overlap. This practical case breaks the base assumption of classic clustering algorithms~\cite{} and makes it infeasible to apply them directly. (2) The PNM data points are not aligned. Even for the non-missing points, the collection period (e.g., caused by delayed response) cannot be guaranteed. Theoretically the standard collection frequency is 1 point per 4 hours. Not surprisingly, in practice, this is only loosely guaranteed. Misaligned data make it challenging to define data points collected at the same collection period among multiple modems for comparison, and thus make clustering challenging. (3) \name must be efficient enough to handle \TODO{XX} TB PNM data. \TODO{Do we have results for performance comparison (ours vs. classic)?} (4) We do not have ground truth to validate the outcome of \name. Only from PNM data, it is impossible to infer the effect to application layer performance. Fortunately, given that ISP's ultimate goal is to improve customer experience, \anonisp provides us another dataset as customer tickets. A ticket is created when a customer called in to report troubles. However, tickets can also be noisy because a customer can call in without networking issues, and many customers also tend to not make a call when the application layer performance is not prohibitively bad. Moreover, a single customer will never be aware of if the problem is a service issue or a maintenance issue. (5) We don't know which metrics are problematic in advance. PNM data have multiple metrics such as \REVIEW{transmission power and receiving power}. Generally speaking, a single outage will only affect a subset of PNM metrics. 

Our main contributions include: (1) We designed and implemented \name, the first system to the best of our knowledge to distinguish maintenance issues and service issues for cable networks. (2) We applied a novel clustering algorithm on the PNM data with missing data points, which introduces cable modems with non-comparable PNM data. (3) We evaluated \name with real world data. \TODO{Our results show that \name saves XX dispatches.} (4) We built the connection between low-level PNM data to high-level application performance and user behavior by analyzing user reported tickets.


==> lessons.tex <==
\section{Lessons Learned}

0. Inferring Missing/lost data is important in network fault diagnosis

1. Can we say that we developed an algorithm  to align data that are collected periodically with missing and unaligned data points?

Think of two more examples that this algorithm might be useful

use case a: Correlate latency to detect congestion events
use case b: performance monitoring in other types of networks:fiber
optic networks, IP, wifi, check pingmesh (xxx)

 - DTW

2.  We found community detetion algorithm works the best in this
scenario. Why spectrum-based mechanism works better than density-based mechanism?

3. Missing data can be helpful in outage detection. Show how many
anomalities are detected using missing.

4.  We developed evaluation metrics that use statistics of noisy
labels to compare the performance of different algorithms. If we
always observe better statistical results from an algorithm, then with
high confidence, we consider it outperforms other algorithms.



% later, after a field trial






==> limitation.tex <==
\section{Limitations and Future Work}

\paragraph{Fine-grained diagnosis} \sys can cluster devices that
share anomalous telemetry data patterns. It can provide hints to where
a fault is located, but cannot provide detailed information as to
which network component causes the fault. This limitation is rooted
from the lack of detailed physical-layer measurement data. When such
data become available, it is possible to extend \sys to become a more
fine-grained diagnosis system. 

\paragraph{Hysteresis} \sys works by analyzing device telemetry
data. It is possible that a sudden network outage (\eg, a cable cut)
occurs before data associated with the outage become
available. Therefore, its time to diagnosis or detection can be behind
a real event. We can mitigate the limitation by more frequent data
collections, but in practice, an ISP has to balance the monitoring
cost and the quality of diagnosis~\cite{yaseen2021towards}.

\paragraph{Customized clustering algorithm} The current implementation
of \sys uses an off-the-shelf clustering algorithm provided by the python-louvain~\cite{python_louvain}
library. It is our future plan to customize the clustering algorithm
to further improve its performance. 

\paragraph{Field experiments} We are in the process of launching field
experiments by deploying \sys at \anonisp. We expect that the results
from the field experiments can realistically evaluate \sys's
effectiveness and how much operational cost it can save. They can also
shed light on further directions of improvement.





==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}



==> old-motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\subsection{Status Quo}\label{sec:status} \jy{ready to read}
PNM best practice document~\cite{cablelabs2016docsis3} written by CableLabs provides an approach to locate different levels of the network issues, such as general plant-wide issues, neighborhood-localized issues, or specific end devices issues, in cable broad networks. This approach uses a clustering algorithm to cluster CMs with similar pre-equalization coefficients. Pre-equalization is a feature in DOCSIS3.0 that allows a CM to use coefficients to pre-distort the upstream signal to compensate for impairments between the CM and the CMTS so that the CMTS will receive signals free of distortion. Therefore, the coefficients provide detailed characteristics of the channel distortion. CMs with the same abnormal pre-equalization coefficients are affected by the same signal impairment. By applying clustering algorithms on pre-equalization coefficients from CMs, ISPs can determine whether a network issue is a service or maintenance issue.

We implemented the recommended algorithm and applied it to our dataset. To evaluate its performance, we use the ticketing rate, an evaluation metric used in CableMon~\cite{hu2020cablemon}, to identify whether network issues detected by the recommended algorithm affect the quality of service (QoS) of cable broadband networks. The ticketing rate means the number of tickets observed in a unit of time. If a fiber optic node served $n$ devices, and during $x$ weeks, the cable ISP received $k$ tickets from % some of the 
customers living in this area, % \zzy{this reads like all $n$ customers must report at least 1 ticket, and customers not reporting tickets are not counted} 
then the ticketing rate is calculated by $k/(n\times x)$. If a network issue exists during a certain period, the ticking rate during this period will increase~\cite{hu2020cablemon}. Normalized ticking rate is defined as the ticketing rate of abnormal periods divided by the overall ticketing rate. We calculate the normalized ticketing rate from the results of the recommended algorithm. The value is only 1.27, indicating that the network issues detected by the recommended algorithm do not highly affect the QoS of cable broadband networks. This surprising result is caused by the design goals of the pre-equalization. The equalizer in each CM adjusts the signal to compensate for the signal impairment during transmission. In many cases, the signal impairment can be mitigated by this feature, which will not directly damage the QoS but affect the pre-equalization coefficients. This helps ISPs find potential issues in the cable network. However, due to the limited resources, our cooperating ISP wants to focus on detecting existing issues that affect customer experience. This inspires us to develop a new tool to detect maintenance and service issues, which can be a complement to the pre-equalization coefficient clustering algorithm.  \zzy{I'm considering whether it is possible that pre-equalization doesn't correlate with QoS because the issue is already repaired by the compensation? If that's true, we may not be able to argue that this recommended method is useless, instead, our work is a complement to it.}


\subsection{Anomaly Patterns} \jy{ready to read}
\label{sec:anomaly}
\begin{figure}[tb!]
\centering
    \includegraphics[width=.45\textwidth]{./figures/pattern_sample.eps}
    \caption{\small\textbf{This figure shows how the  transmission
        power of six cable devices in the same fiber optic node
        fluctuate over time.}}
    \label{f:tx_power_examples}
\end{figure}

\begin{figure}[tb!]
\centering
    \includegraphics[width=.45\textwidth]{./figures/pattern_sample_map.eps}
    \caption{\small\textbf{This figure shows the locations of the
        cable devices using colored dots. Orange dots are devices that
        show the same anomalous transmission power patterns. Green
        dots are devices that show normal patterns. Red dots are
        devices that show distinct anomalous patterns. }}
    \label{f:tx_power_examples_map}
\end{figure}


Instead of focusing on pre-equalization coefficients, we checked all the metrics mentioned in Section~\ref{sec:dataset}. We manually examined several anomaly patterns to gain insights into how to separate a service issue from a maintenance issue. Figure~\ref{f:tx_power_examples} shows an example. In this figure, we sampled the transmission power levels of devices with three anomaly patterns from a fiber optic node. The orange dots show the transmission power levels of three devices that exhibit similar anomalous patterns in the changes of their transmission powers. When a noise leaks inside a cable transmission channel, a device increases its data transmission power to overwhelm the noise. So a sudden increase in transmission power is an indicator of noise invasion. The green dots show the transmission power levels of two devices that are not impacted by the noise. The red dots show the transmission power levels of a device that exhibits a different anomalous pattern.

Figure~\ref{f:tx_power_examples_map} shows the geographic distribution
of the devices in the fiber optic node. We use the same color coding schemes
to plot the devices. The orange dots plot the geographic locations of
the devices that exhibit similar anomalous patterns as depicted in
Figure~\ref{f:tx_power_examples}. Each red dot shows the geographic
location of a device that exhibits a distinct anomalous pattern. And
the green dots show the locations of the devices that do not exhibit
any anomalous pattern.

We highlight two observations. First, we observe that there is a red
dot located within the orange cluster. Without an automated algorithm
that classifies the anomalies into two distinct patterns, an operator
may erroneously conclude that the device depicted by that red dot
was affected by the same network issue as the devices depicted by the
orange dots. Second, we observe that the transmission power levels of
the three devices in orange dots have different values, but the
increase and decrease trends are common. Similarly, those of the two
devices in green dots have different values, but are both flat with
small fluctuations. This observation motivates us to use a clustering
algorithm to group devices that exhibit similar anomalous behaviors
together. The hypothesis is that similar anomalous patterns are a
strong indicator that the devices are affected by a common fault in
the network. Therefore, we can conclude that the fault is a
maintenance issue. In contrast, a distinct anomalous pattern as
depicted by the red dots in Figure~\ref{f:tx_power_examples} suggests
there exists a different network fault without widespread effects.
% that affects only a small number of customers. \zzy{Do we mention that we consider clusters with size under 5 as service issues? If so, it may be against the statement here.}


% we also observe that
% devices may exhibit the same anomalous trends in their PNM values, but
% the absolute values of the metrics can differ.

% 
% 
% of a maintenance issue. The figure plots the transmission powers of
% five sampled devices residing in the same fiber optic node. The
% transmission power patterns of two devices are flat, while three of
% them show a similar abnormal pattern: the transmission powers of the
% three devices remain high for a period of time and then decrease. When
% a noise invades the transmission channels of a network, devices
% increase their transmission powers to increase the signal-to-noise
% ratio of their transmitted data. So the sudden increases of multiple
% devices' transmission powers are a reliable signal that a noise has
% entered the network and affected a shared segment of the network.
% 
% 
% \xy{Jiyao, can we add a service issue here?} 
% 
%  first, then decreases. Therefore, by applying clustering
% algorithms on different patterns of each PNM metric, we can
% distinguish the unhealthy modems from the healthy ones. However, there
% are three challenges we need to solve compared to applying the
% traditional clustering algorithms to our data directly.
% 
% 
% From our data, we
% further observe that the modems affected by the same network faults
% often show similar abnormal patterns.
% 
% indicating that these two modems work well. Modem 3, 4, and 5




==> old_evaluation_method.tex <==
% \subsection{Overview}

% from the devices in the same fiber optic node

\sys's main goal is to separate maintenance issues and service issues. In this section, we evaluate how well \sys meets this goal by answering the following research question (RQ): \textbf{RQ1: } \emph{When \sys diagnoses that a network anomaly is caused by a maintenance issue, how often it is indeed a maintenance issue?} (\S~\ref{sec:ticketing_rate}) We evaluate the effectiveness of \sys using both labeled data and tickets. Besides, we are also interested in understanding how a common network fault impacts devices and subscribers. For example, \textbf{RQ2: } \emph{What is the average time for a maintenance or service issue to be fixed?} (\S~\ref{sec:ticket_characteristics}) \textbf{RQ3: } \emph{How often do subscribers report such faults?} (\S~\ref{sec:result_stats}) We will show our answers in this section in order. 
  
\subsection{Methodology}
\jy{ready to read}
\label{sec:eval_method}
It is challenging to evaluate \sys's effectiveness due to the lack of ground truth. We develop a method that combines manual labeling and trouble ticket statistics to gain insight into \sys's effectiveness. 

\paragraph{Manual Labeling} We manually labeled a small set of data as ground truth for evaluating \sys. We visually examined the telemetry data in a format similar to Figure~\ref{f:tx_power_examples} in a certain time period. We use customer trouble tickets to help us locate such periods. If a group of devices shows a common anomalous pattern, we label this group of devices affected by a network fault. If the group size is larger than 5, we label this network fault a maintenance issue. Otherwise, we label it as a service issue. We learned from \anonisp's industry experts that this process resembles how they manually diagnose a network anomaly. 

We started the inspection by choosing over 50 primary tickets (\ie, tickets that can reflect maintenance issues) \zzy{maybe add a ptr here as primary ticket is already defined in the dataset section} and used the tickets' start and close time to guide the search for anomalous patterns. We are able to obtain 16 groups of maintenance issues that impact nearly 700 devices. Since we must inspect all devices sharing the same \FN for each primary ticket, we were also able to identify 113 devices that were affected by service issues. We carefully verified the labeling results with \anonisp's experts to guarantee the labeling accuracy.%This manual labeling process is tedious and prohibitively expensive: we spent nearly one week of work time to obtain these labels. \zzy{I'm wondering if we should mention this... As 1 week doesn't sound too bad. I understand you're trying to explain the reason why the dataset is small, then I think only mentioning to "guarantee the labeling accuracy" is sufficient.} We intentionally did not expand into more labels to guarantee the labeling accuracy.

\paragraph{Trouble Ticket Statistics} We use trouble ticket statistics as a more scalable approach than manual labeling to evaluate \sys's effectiveness. According to \anonisp's operational experience, although dispatch decisions are sometimes incorrect, the necessary dispatch decisions still outnumber the incorrect ones. \zzy{Have we verified this with wade? I could be wrong but I don't remember this conclusion.}\jy{I think Wade mentioned nearly 40\% are wrong} Therefore, if \sys correctly diagnoses the root cause of an anomaly, then on average, we should observe that there are more maintenance tickets than service tickets during the anomaly events diagnosed as maintenance issues and vice versa. Similarly, because a maintenance issue impacts users differently compared to a service issue, if \sys correctly diagnose an anomaly, we should observe different ticket statistics for a maintenance issue and a service issue, respectively. Therefore, we use the normalized ticketing rate to further gauge \sys's effectiveness.

In \S~\ref{sec:deploy}, we mention ISPs can run \sys in two modes: \reactive and \proactive. We evaluate both modes using trouble ticket statistics. % \zzy{Now this is the first occurrence.} 
For the \proactive, we invoke \sys daily on each \FN. Suppose we invoke \sys on time $t$, we run \sys using the \pnmdata collected between $t - 1$ day and $t$ among all devices in the same \FN. We then use a single-device diagnosis tool such as CableMon to diagnose whether each cluster that \sys output indicates a service issue, maintenance issue, or no issue. For the \reactive, if a customer trouble ticket is reported at time $t$, and the network’s single-device diagnosis tool signals that there is a hardware-related anomaly on the ticket-associated device, we run \sys among the \pnmdata collected between time $t - 1$ day and $t$ among all the devices in the same \FN. The cluster that the abnormal device belongs to indicates a service issue or maintenance issue, which can be determined using the size of the cluster. Finally, we calculate the corresponding trouble ticket statistics on both \reactive and \proactive. 


 % \zzy{we may better to use FN and fiber optic node more consistently}\jy{I think we should always use the fiber optic node instead of FN in this paper, since false positive is also FN} \zzy{+1}
 


\paragraph{Comparison} We made the design choice of using the average-linkage hierarchical clustering algorithm. To evaluate this design choice,  we compare \sys with three other clustering algorithms: DBSCAN~\cite{ester1996density}, single-linkage hierarchical clustering~\cite{sibson1973slink}, and complete-linkage hierarchical clustering~\cite{defays1977efficient}. All these clustering algorithms have hyper-parameters. We use a grid search method~\cite{bergstra2012random} to tune those parameters, including the similarity threshold $s$ parameters used by \sys (\S~\ref{sec:clustering}). Specifically, for each clustering algorithm, we choose the values of the hyper-parameters that maximize the normalized maintenance ticketing rate. The normalized ticketing rate is defined in \S~\ref{sec:status}. \zzy{This is defined afterwards (the paragraph titled "Normalized ticketing rates"). Should we move this paragraph behind the definition?} The normalized maintenance ticketing rate is the rate that only considers primary tickets during the calculation. \zzy{Now we have 2 sets of definitions, although they are equivalent: one defined normalized maintenance ticketing rate from scratch (the paragraph titled "Normalized ticketing rates"), another derived from normalized ticketing rate (here). I feel like the one derived from plain ticketing rate is easier to understand.}



\paragraph{Normalized ticketing rates} Ticketing rate is the number of
trouble tickets an ISP receives per unit time. \zzy{There is a gap between plain ticketing rate and maintenance/service ticketing rate. This intuition does not fit the notations below well.}  Support \zzy{Suppose?} a
device $x$ experiences a network anomaly event $e$. If the
anomaly event lasts for a time period $t_{e,x}$, and during this time
period, an ISP receives $k_{e,x}$ tickets from the subscriber of
device $x$. We refer to it as ``the event $e$ \emph{captures} the
$k_{e,x}$ tickets.'' If there are no tickets reported by any subscriber,
then $k_{e,x} = 0$. \sys will diagnose an anomaly event $e$ as either
a maintenance issue or a service issue. And a ticket can either be a
maintenance ticket or a service ticket.  Let $T_k$ denote the type of
a ticket and and let $T_e$ denote the type of a diagnosed event. We
can define four types of ticketing rates $R_{T_k, T_e}$ as the total
of number of type $T_k$ tickets by the sum of the $T_e$ event lengths:
$R_{T_k, T_e}
= \sum_{x,\{e|T_e\}} \frac{\{k_{e,x}|T_k\}}{t_{\{e|T_e\}},x}$. We
define a baseline ticketing rate $B_{T_k}$ for a ticket type $T_k$ as
the total number of type $T_k$ tickets divided by the entire data
collection period. A normalized maintenance/service ticketing rate is
the maintenance/service ticketing rate divided by the baseline
maintenance/service ticketing rate.

\zzy{Now the definition in \S\ref{sec:set_similarity_threshold} becomes a special case of this definition. But we do not connect them in any way in the text. I would recommend to either (1) have the more general definition (here) and then use it in a specific case (\S\ref{sec:set_similarity_threshold}) or (2) use the special case first and then introduce more general def (here), as we're doing now, but clarify how it can be specific to the previous specific case (\S\ref{sec:set_similarity_threshold}).}

\if 0

our clustering algorithm. However, evaluating the
performance of clustering algorithms is
difficult~\cite{pfitzner2009characterization}. There are two concrete
approaches evaluating the results of clustering algorithms: external
criteria and internal criteria~\cite{halkidi2001clustering}. Both of
them have intrinsic limitations that prevent us from deploying them on
a large scale. External criteria need labeled data as ground truth and
compare the clustering results with ground truth. However, labeling
data as ground truth requires significant human efforts, and relies on
expert knowledge to determine whether different vectors belong to the
same cluster. Our data contains 77,696 devices from 394 \FNs, which
makes impractical for us to label enough ground truth over the entire
dataset to evaluate the performance of clustering algorithms. Internal
criteria aim to use the clustering result itself to evaluate the
performance of clustering algorithms. It measures the similarity
between all the vectors inside the same cluster. However, it cannot
infer the physical meaning, \ie, whether the clustering result
captures maintenance issues and service issues.
%, which still requires a reasonable evaluation metric. \zzy{I don't get this statement, what do you mean?}
% However, a concrete evaluation metric is still



This section introduces how we demonstrate the effectiveness of \sys with the consideration of the intrinsic difficulty of evaluating clustering results. We aim to answer the following research questions (RQs) as our roadmap for evaluation:

\begin{itemize} [topsep=0.1ex,leftmargin=2\labelsep,wide=0pt]
        \setlength\itemsep{0em}
\item \textbf{RQ1 (Section~\ref{sec:manual_label}):} \emph{How precisely can we reproduce experts' investigation?} 
\item \textbf{RQ2 (Section~\ref{sec:ticketing_rate}):} \emph{How accurately can we detect maintenance issues that match the customer report tickets?}
\item \textbf{RQ3 (Section~\ref{sec:result_stats}):} \emph{Are there any characteristics of the customers affected by maintenance issues as a guidance for ISPs to label tickets more accurately?}
\item \textbf{RQ4 (Section~\ref{sec:efficiency}):} \emph{Is it feasible for an ISP to perform maintenance issue detection without a large-scale cluster?} 
\end{itemize}

\fi

% To overcome the difficulty for evaluation, we firstly conduct a small-scale study using external criteria based on a set of manually labeled samples (Section~\ref{sec:manual_label}). Then we perform a large-scale experiment with the help of customer report tickets (Section~\ref{sec:ticketing_rate}). We aim to answer the research question as: \emph{Can maintenance issues detected by \sys match the tickets reported by customers?} In Section~\ref{sec:result_stats}, we reveal the characteristics of the detection results by deeply analyzing the statistics. The section resolves the following research questions: \emph{How does the group of customers affected by one maintenance issue distribute geographically?} \emph{Do customers tend to report tickets when they are affected by a maintenance issue?} \emph{To what extent does an ISP label tickets as maintenance tickets incorrectly?} Last but not least, in Section~\ref{sec:efficiency}, we studied the research question as \emph{Is it feasible for an ISP to perform maintenance issue detection without a large-scale cluster?} \jy{I think too many emph is hard to read}



==> old_ticketing_rate.tex <==
\subsection{Ticket-Based Evaluation}
\label{sec:ticketing_rate}

Since we only have a small set of manually labeled data, we resort to using ticket statistics to estimate \sys's clustering on a larger scale in both \proactive and \reactive. We should each result in sequence.

\subsubsection{\PROACTIVE}
\label{sec:proactive}
For the \proactive, we simulate the way that \anonisp will use \sys, which will invoke \sys daily on each \FN, to diagnose whether an anomaly event experienced by a device is a maintenance issue or a service issue. We then compute the normalized maintenance ticketing rate and the normalized service ticketing rate for events diagnosed as maintenance issues. Similarly, we compute the normalized service ticketing rate and the normalized maintenance ticketing rate for events diagnosed as service issues. If we assume the ticket type labeled by an operator is mostly correct, and if \sys separates maintenance issues from service issues with high accuracy, we expect to see a much higher normalized maintenance ticketing rate than the service ticketing rate for maintenance issues and vice versa for service issues. Therefore, we adopt four types of normalized ticketing rates as the evaluation metric in this subsection.

\begin{table}[h]
\scriptsize
\centering
\begin{tabular}{c c c c c}
%\toprule
         & \multicolumn{2}{c}{Maintenance Issues} & \multicolumn{2}{c}{Service Issues} \\\cmidrule{2-5}
         & \makecell[c]{Maintenance \\ Tickets}  & \makecell[c]{Service \\ Tickets} & \makecell[c]{Service \\ Tickets}  & \makecell[c]{Maintenance \\ Tickets}\\ \midrule
SNR         &  xx     & xx  & xx & xx        \\ \midrule
Txpower     &  xx     & xx  & xx & xx        \\ \midrule
Missing     &  xx     & xx  & xx & xx          \\ 
\midrule
Combined    &  xx     & xx  & xx & xx         
% \bottomrule
\end{tabular}
\caption{\textbf{\jy{Results of training data}\label{tab:our_ticket_density_train}}}
\end{table}

\begin{table}[h]
\scriptsize
\centering
\begin{tabular}{c c c c c}
%\toprule
         & \multicolumn{2}{c}{Maintenance Issues} & \multicolumn{2}{c}{Service Issues} \\\cmidrule{2-5}
         & \makecell[c]{Maintenance \\ Tickets}  & \makecell[c]{Service \\ Tickets} & \makecell[c]{Service \\ Tickets}  & \makecell[c]{Maintenance \\ Tickets}\\ \midrule
SNR         &  7.12     & 3.30  & 7.33 & 6.79        \\ \midrule
Txpower     &  3.10     & 2.02  & 3.83 & 1.96        \\ \midrule
Missing     &  6.86     & 2.67  & 13.00 & 2.63          \\ 
\midrule
Combined    &  4.28     & 2.40  & 8.01 & 2.02         \\ \midrule
\makecell[c]{Pre-equalization \\ Coefficients} & 1.52 & 1.37 & 1.36 & 1.31
% \bottomrule
\end{tabular}
\caption{\textbf{The values of different types of
    normalized ticketing rates based on 
    \sys's diagnosis result in \reactive.\jy{TODO: add ticket density for normal groups as well}\label{tab:our_ticket_density}}}
\end{table}

\begin{figure}[h]
\centering
    \includegraphics[width=.45\textwidth]{./figures/our_ticket_density.eps}
    \caption{\small\textbf{} \zzy{Redraw fig of table~\ref{tab:our_ticket_density}. Pre-Equal stands for pre-equalization coefficients.} \zzy{TODO: $NTRR_*$ is not defined}} 
    \label{f:our_ticket_density}
\end{figure}


We split the \pnmdata collected between 01/06/2019 and 11/30/2019 as a training set, and the \pnmdata collected from 12/01/2019 to 02/28/2020 as a test set. We find the best Clustering similarity threshold $s$ on our training set for each feature individually and use the test set to validate the effectiveness of \sys. Besides, we also show a comparison between \sys and the pre-equalization coefficient clustering algorithm recommended by CableLabs~\cite{}. 

Table~\ref{tab:our_ticket_density} shows the results when we run \sys in \reactive. We list the ticketing rates for anomalies detected by each independent feature. The ticketing rates listed in the ``combined'' row combine the anomaly events detected by all features. For events diagnosed as maintenance issues, \sys's normalized maintenance ticketing rate is much higher than the normalized service ticketing rate for all features individually and the combined result. For events diagnosed as service issues, \sys's normalized service ticketing rate is higher than the normalized maintenance ticketing rate for all features individually and the combined result, but the difference between them for the SNR feature is small.  We note that the normalized service ticketing rate is as high as $13.00$, suggesting that missing data collection points is highly predictive of service issues. 

\if 0
\begin{table}[h]
% \scriptsize
\centering
\begin{tabular}{c c c c c}
% \toprule
            & \sys & DBSCAN & \makecell[c]{Single \\ Linkage}  & \makecell[c]{Complete \\ Linkage} \\ \toprule
SNR         & 8.54          & 5.39  & 6.50  & 7.00        \\ \midrule
Txpower     & 4.16          & 2.21  & 2.61  & 3.26        \\ \midrule
Missing     & 3.76          & 3.34  & 3.79  & 3.62         \\ \midrule 
Combined    & 3.95          & 2.65  & 2.98  & 3.31         \\ % \bottomrule
\end{tabular}
\caption{\textbf{Normalized maintenance ticketing rate for maintenance issues detected by different algorithms in \reactive.}\label{tab:normalized_ticketing_rate}}
\end{table}

Table~\ref{tab:normalized_ticketing_rate} shows the normalized maintenance ticketing rate for the maintenance issues detected by each performance metric among \sys and other clustering algorithms. This result indicates whether the customer reports more tickets during the maintenance issues each algorithm detected. From this table, we can observe that \sys achieves the highest normalized maintenance ticketing rate among all the algorithms we compared. For the maintenance issues detected by missing, the performance of \sys, single-linkage and complete-linkage hierarchical clustering algorithm is similar since missing contains less noise compared to other metrics. \zzy{Does that imply \sys's advantage is mainly to overcome noise? Otherwise why is the performance similar because of less noise?} 

We also compared the other three types of ticketing rates between \sys and
other clustering algorithms. Due to the space limit, we present the
results in Appendix~\ref{appendix:tables}. The results show that \sys consistently
outperforms other clustering algorithms.
\fi

\subsubsection{\REACTIVE}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\begin{tabular}{cccc}
% \cline{3-4}
&             & \multicolumn{2}{c}{Ticket Label}          \\ \cline{3-4} 
&             & M & S \\ \cline{2-4} 
\multicolumn{1}{c}{\multirow{2}{*}{\makecell[c]{\sys's \\ Diagnosis}}} & M & 2147 ($TP$)       & 1062 ($FP$)    \\ \cline{2-4} 
\multicolumn{1}{l}{}                                                                        & S     & 175 ($FN$)        & 1168 ($TN$)    \\ % \hline
\end{tabular}
\caption{\textbf{Confusion Matrix for Ticket Type. ``M'' denotes ``Maintenance'' and ``S'' denotes ``Service''.}\label{tab:confusion_matrix}}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{cccc}
% \cline{3-4}
&             & \multicolumn{2}{c}{Ticket Label}          \\ \cline{3-4} 
&             & M & S \\ \cline{2-4} 
\multicolumn{1}{c}{\multirow{2}{*}{\makecell[c]{\sys's \\ Diagnosis}}} & M & 362 ($TP$)       & 260 ($FP$)    \\ \cline{2-4} 
\multicolumn{1}{l}{}                                                                        & S     & 35 ($FN$)        & 293 ($TN$)    \\ % \hline
\end{tabular}
\caption{\jy{Results for Test Set}\label{tab:test_set_data}}
\end{table}

We also evaluate the effectiveness of \sys in the \reactive. We invoke \sys when a customer trouble ticket arrives and the network's single-device diagnosis tool signals this ticket is associated with a hardware-related network issue. \sys will output whether this network issue is a service issue or a maintenance issue. We use this result to predict the arrived ticket as a service ticket or maintenance ticket. We then compare our prediction results with the ticket type labels provided by the operator. If we assume that the ticket type assigned by an operator is mostly accurate and \sys can effectively distinguish between maintenance issues and service issues, we should observe significantly higher correctness of prediction results on both maintenance tickets and service tickets.

Table~\ref{tab:confusion_matrix} shows the comparison between our prediction and the ticket type labels. Among all the 2,322 maintenance tickets, \sys successfully predicts 92.46\% of them are triggered by maintenance issues. Meanwhile, \sys reports there are 3,209 tickets associated with maintenance issues, where 66.90\% of them were labeled as maintenance tickets by the \anonisp. This result follows the observation from \anonisp that the maintenance team mislabeled more maintenance tickets as service tickets, and sent them to different teams to fix, which will lead to redundant dispatches, incremental operational costs, and worse customer experience.
If we assume the output of \sys is correct, then we can save nearly 30\% of wrong dispatches. \jy{I am not sure whether we should mention it here or in section 6.5}


\paragraph{Summary:} We observe salient statistical differences between ticketing statistics when \sys diagnoses an anomaly event as a maintenance issue or as a service issue. This analysis provides evidence that \sys can effectively separate maintenance issues from service issues.




==> parameters-old.tex <==
\subsection{Parameter Settings}\jy{should be removed}
\label{sec:parameters}

The \sys design has five tuneable parameters. We describe how to set
those parameters in turn.

\begin{itemize} [topsep=0.1ex,leftmargin=2\labelsep,wide=0pt]
        \setlength\itemsep{0em}
\setlength{\itemsep}{0pt}
\setlength{\parskip}{0pt}
\item $d$: the lookback days of a device's telemetry data. How to set
  $d$ depends on several factors, including the telemetry data
  collection frequency, how many data points are sufficient for
  computing similarity scores between two devices, and what fraction
  of data points are missing. For the datasets we have, we find one
  week of data works well. The data we have are collected from three
  adjacent RF channels every four hours. So on average, each device
  has $6 \times 7 \times 3 = 126$ data points. For ISPs that use
  different data collection intervals or different numbers of RF
  channels, we hypothesize that as long as the value of $d$ ensures that there
  are $100+$ data points, \sys would work well.

\item $c$: the minimum number of devices in an anomalous cluster for a
  fault to be diagnosed as a maintenance issue. We set this value to
  five in \sys, based on the feedback from \anonisp's industry
  experts that most maintenance issues impact no fewer than five
  devices.

\item $o$: the minimum number of overlapping data points for two devices to be
  comparable. We set this value to be one third of the expected number
  of data points collected in $d$ days in a device's telemetry
  data plus one, since ~\cite{hu2020cablemon} detects abnormal events when 2/3 of data points show anomalies. This value can ensure we have at least one abnormal data point overlapped. For the datasets we have, we set $o$ to $126 \times 1/3 + 1 = 43$.

\item $s_f$: the minimum similarity score for creating an edge between
  two devices to generate the input graph for the Louvain algorithm
  (\S~\ref{sec:clustering}) for feature $f$. We tune this parameter by
  performing a grid search guided by the trouble ticket statistics. We
  describe the process in more detail in
  \S~\ref{sec:eval_method}.

\end{itemize}

  


==> rational.tex <==
\subsection{Design Rationale}\label{sec:rationale}

We aim to use clustering algorithms to cluster the modems affected by the same network fault.


First, the time series data among different modems in the same fiber optic node are not aligned. Since we aim to cluster the modems that show abnormal patterns at the same time, the unaligned time between different modems may make the similarity calculation inaccurate. Therefore, we need an algorithm to align the data collection time among all the modems in the same fiber optic node. \zzy{I'm considering if this is a specific challenge for clustering? What if people are asking "does previous work (cablemon) also need alignment?"}\jy{Only when we compare different modems will we need this align algorithm. For cablemon, we just focus on each individual modem} %Therefore, in order to utilize the missing as an availability metric to detect the network faults, we must infer where the missing data points are in our data set.

Second, our data set contains missing data points. According to ~\ref{xx}, our PNM data will be collected every 4 hours. However, since the SNMP protocol is built on UDP, sometimes we cannot receive responses from a target cable modem due to various reasons, such as network congestion, cable broken, and power off. This no-response issue will not be recorded in the PNM data given the design of the data collection framework. From Figure~\ref{f:tx_power_examplese}, we could observe that both modem 3 and modem 4 contain missing data points, which are shown in red dots. Since different modems may contain different amounts of missing data points, the dimension of the input vectors of different modems may vary, which brings obstacles to calculating the similarity between different time series data.

Finally, some modems' time series data do not overlap with each other, which makes it impossible for us to calculate the similarity between these two modems. For example, in Figure~\ref{f:design_rationale}, modem $x$ has no valid data points overlapped with valid data points from modem $y$, which makes these two modems incomparable. Most of the clustering algorithms require calculating pairwise similarity/distance for all pairwise nodes, making them unsuitable for applying to our data set.

Dynamic time warping (DTW)~\cite{sakoe1978dynamic} is an algorithm to align time series data before establishing distance measurements. However, we do not adopt this algorithm to solve the first and second challenges due to the following reasons: First, DTW uses amplitude similarity to align the time series data. In our work, we only need to align the data points with the closest data collection time. Second, DTW is not efficient. Its time complexity to calculate the aligned time among two vectors is $O(N^2)$ if the length of each vector is $N$. One of our goal is to design a more efficient algorithm.

In this section, we will first describe our time series align algorithm with high efficiency in Section~\ref{sec:align}. We then describe how we select the similarity measurement metric that works for the data set with missing data in Section~\ref{sec:distance}. Finally, in Section~\ref{sec:cluster}, we present the clustering algorithm we used to cluster the modems that are affected by the same network fault when some time series data are not comparable.
%Finally, we introduce how we can
%find the possible location of the networking faults by using the clustering results we achieved in the previous step.


==> related.tex <==
\section{Related Work}
\label{sec:related}
% Fault diagnosis is important to any network service providers.
% In this section, we
% summarize related work and how it relates to this work.

Both Volpe \ea~\cite{volpe2021machine} and the PNM best practice
document~\cite{cablelabs2016docsis3} propose to use a clustering
algorithm to separate maintenance issues from service issues. Volpe
\ea propose to use an outlier detection algorithm on Full Band Capture
(FBC) data, which is another type of telemetry data that can be
collected by the PNM infrastructure  and apply
DBSCAN~\cite{ester1996density} to group cable devices sharing the same
anomalous patterns for reducing operational costs caused by erroneous
dispatches. However, the authors acknowledge in their work that there
are no good approaches to tune the hyper-parameters of the system and
the work does not include the experimental evaluation of the effectiveness
of using FBC data as features and the parameter settings of the
outlier detection and DBSCAN clustering algorithm. The PNM best
practice document proposes to use pre-equalization coefficients as
feature vectors for clustering. Similarly, there is no evaluation of
how well the proposed system works. Moreover, this previous work does
not address the data incompleteness and alignment issues caused by
unreliably collected data in production systems.

% the work provides a visualization tool to help human operators observe
% groups of devices sharing similar FBC data patterns without providing
% any numerical evaluation results.

\sys uses a different set of PNM features (SNR, Tx power, and missing
data points) for clustering. By utilizing customer
 tickets and operational knowledge, it programmatically
optimizes all hyper-parameters to adapt to different ISPs' operating
environments. In addition, it does not need manually labeled
data. Moreover, we implement \sys and evaluate its performance to show
its effectiveness. We have also compared \sys with
pre-equalization-coefficients-based fault diagnosis in
\S~\ref{sec:ticketing_rate} and show that \sys's features are more
effective at detecting customer-impacting faults.

Our \pnmdata do not include FBC data. There is also rich work in the
literature proposing to add new metrics in the PNM
infrastructure~\cite{campos2018proactive,jones2022amplifier,hranac2022docsis}.
\sys is orthogonal to this body of work, and we believe \sys's
architecture, its methodology to avoid labeled data and hand tuning,
and its data pre-processing techniques can be extended to a broader
set of \pnmdata.

Fault detection in cable broadband networks has been widely
studied~\cite{lartey2017proactive,rupe2019kickstarting,cablelabs2016docsis3,keller2019proactive,zhou2020proactive,hu2020cablemon,ferreira2020convolutional}. \sys
tackles a different problem: how to diagnose a fault. \sys can use any
fault detection system that meets the following requirements: is
effective, does not use labeled data, and does not need to hand-tune
hyper-parameters. It incorporates CableMon~\cite{hu2020cablemon} as
its fault detection system, as CableMon meets these design
requirements. However, unlike \sys, CableMon cannot diagnose the fault
type. Other methods either use hard-coded
thresholds~\cite{lartey2017proactive,rupe2019kickstarting,cablelabs2016docsis3,keller2019proactive,zhou2020proactive}
for anomaly detection or use manually labeled training data for
classification~\cite{ferreira2020convolutional}.
 
\if 0
The cable industry has actively explored approaches using PNM data for
fault diagnosis.  The publicly known best current practice is to
detect network anomalies with hard-coded
thresholds~\cite{lartey2017proactive,rupe2019kickstarting,cablelabs2016docsis3,keller2019proactive,zhou2020proactive}.
 
For example, Rupe \ea~\cite{rupe2019kickstarting} propose to monitor a series of PNM metrics such as uncorrectable codewords and raise an alarm if a monitored metric exceeds a fixed threshold, \eg, uncorrectable codewords are higher than 0.1\% for over an hour.
Previous work~\cite{keller2019proactive,zhou2020proactive} also applied hard-coded thresholds onto different metrics or features other than the ones we are using in this work. Keller \ea~\cite{keller2019proactive} monitor CMTS trap messages as an indicator of CMs being online/offline. The system signals an anomaly when the number of offline CMs exceeds a pre-defined threshold longer than a pre-defined time period.
Hard-coded thresholds highly depend on operators' experience and there is no guarantee that the threshold can be applied to other networks or even the same network at different time periods. In contrast, 
\name
can automatically tune an optimal machine learning model
for different networks, and adaptively update the underlying model over time to overcome model drift by using customer tickets to guide model construction. \PENDING{CableMon~\cite{hu2020cablemon} introduces adaptive threshold to detect anomalies, however, unlike \name, it cannot tell the fault type.}

Ferreira \ea~\cite{ferreira2020convolutional} proposed to use a convolutional neural network model to detect cable network anomalies. They use the amplitudes of a CMTS received signal as features and a manually-labeled dataset for training. The model also requires defining anomaly categories in advance. The features they use are similar in nature to the pre-equalization coefficients that we compare with in \S~\ref{sec:ticketing_rate} and are not as effective as the features \name uses in indicating real-world network impairments. In addition, \name uses unsupervised learning and does not require manual labels.
\fi

% \zzy{I still thin pre-defined category required by the CNN work is a huge drawback that we should mention.}
% \sout{
% CNN model for clustering. However, as a supervised learning model, the model needs manually labelled dataset and also requires defining the anomaly categories in advance. \name does not have such requirements. 
% }

There exist tools that aim to assist ISPs' manual troubleshooting by
offering visualization and suggestions to
operators~\cite{milley2019proactive,rupe2020profile,volpe2021machine,walsh2009pathtrak}. \sys
aims to automate fault diagnosis and can be enhanced with a graphical
user interface.

% aims to  
% Rupe \ea~\cite{rupe2020profile} proposed to calculate a severity indicator from Receive modulation error ratio (RxMER), which helps operators prioritize repairing CMs with the highest severity.
% We also learnt from \anonisp that the cutting-edge industrial tool is Pathtrak~\cite{walsh2009pathtrak}. The tool analyzes pre-equalization coefficients, and provides UIs for operators to manually inspect potential faults.
% 


% \paragraph{Clustering algorithms for anomaly detection}

% Wu \ea~\cite{wu2016survey} classified the anomaly
% detection algorithms into five categories according to the detection
% criteria: based on statistical, clustering, deviation, distance and
% density. 

% \xy{I still think we can move this part somewhere else. i think we can comment out this  for now.}
% \textbf{Time series alignments.}
% Alignment is a well-known issue for time-series data, which \name consumes. 
% Dynamic Time Warping (DTW)~\cite{dtw94berndt} is a 
% popular alignment algorithm that measures the similarity between two time series data with time warping. However, it is not suitable for our work % for two reasons. Firstly,
% because
% it uses values of metrics to align the time series data based on the assumption that the two time series data may have different phases. However, in our work, we observe all the metrics changing at the same time when there is a maintenance issue. % Secondly, the time complexity of DTW is $O(N^2)$. \sys requires a more efficient alignment algorithm for achieving efficiency.

% zzy: Remove clustering on non-PNM data to save space
% \textbf{Clustering for anomaly detection.}
% Researchers have applied clustering algorithms % \st{have been proposed}
% for detecting anomalies on
% time series data~\cite{zhang2016taskinsight,
%   li2021clustering}. Ferreira \ea~\cite{ferreira2016time} compared the
% performance of community detection algorithms with other clustering
% algorithms for clustering time series data.
% Cao \ea~\cite{cao2014uncovering} use a hierarchical-clustering
% algorithm to scalably detect groups of fake accounts that act
% together, which is a signature of bot accounts. Botminer~\cite{gu2008botminer}
% uses X-means~\cite{pelleg2000x} to cluster machines that exhibit similar
% behaviors and classify them as bots. Different from previous work, we developed pre-processing techniques to align data collected at different points in time and use missed data collection points as a feature to detect network unavailability. 


% \sout{Differently, we use a community
% detection algorithm for diagnosing the type of fault in cable
% broadband networks. The clustering algorithm may partition a network
% of devices into several groups, and \sys depends on an anomaly
% detection system to determine whether a group is anomalous or not.}

% Another use case of clustering-based anomaly detection is fake account
% detection in Online Social Networks. Previous
% work~\cite{cao2012aiding, cao2014uncovering} reveals the effectiveness
% of applying clustering algorithms onto social networks to recognize
% accounts with abnormal behavior patterns as fake accounts. \name
% shares similar ideas for clustering with this previous work but also
% faces unique challenges for the \pnmdata coming from cable
% networks. For example, as a result of the unreliable transmission
% protocol, missing points caused by packet loss are common while the
% studies for Online Social Networks do not have this challenge.

% to pinpoint root causes by finding the


% \zzy{Delete this paragraph?} SNAP~\cite{yu2011profiling} collects TCP statistics and socket-level
% logs and then uses Pearson correlation among a collection of flows'
% statistics to detect performance anomalies. Differently, \sys uses
% Pearson correlation as a similarity metric used by a clustering
% algorithm.

% it also uses a clustering algorithm to group cable devices that share
% similar anomalous data patterns.
% % 
% similarity for clustering but unlike SNAP, which can only produce a
% binary output as normal or abnormal, \sys can tell apart multiple
% maintenance or service issues simultaneously.


% \name's clustering algorithm is similar to the proposed algorithm but
% has also been elaborately adjusted for the challenges raising by cable
% networks such as data alignment.

% Time series clustering using community detection: ~\cite{ferreira2016time}

% using clustering to detect anomaly: ~\cite{zhang2016taskinsight, li2021clustering}

% a survey on anomaly detection on time series data ~\cite{wu2016survey}


% \textbf{Customer tickets in network troubleshooting.}  
Researchers and
practitioners have used customer tickets for network
troubleshooting. NetSieve~\cite{potharaju2013juggling} analyzes
natural language text in customer tickets to automate root cause
analysis. LOTUS~\cite{venkataraman2018assessing} analyzes natural
language text in customer tickets to estimate the impact of network
outages. CableMon~\cite{hu2020cablemon} uses customer tickets as hints
to set anomaly detection thresholds in cable broadband networks. This
work is inspired by CableMon's techniques of adaptively choosing
anomaly thresholds  and does not use the natural
language text in customer tickets for design simplicity. 

% \zzy{nit: CableMon
%   doesn't use natural language.}  Instead, it uses customer ticketing
% rate statistics to guide feature selection and to tune the
% hyper-parameters of an unsupervised machine learning model.

% \sys diagnoses the type of fault that causes an anomaly and can work with CableMon or other anomaly detection systems. \xy{cablemon is not a clustering algo. should be moved to the anomaly detection sub-section.} \zzy{But this paragraph is not for clustering. It's for approaches based on tickets. I mentioned it in both paragraphs.}


% \zzy{Do we need any comparison with CableMon?}
% \st{as evaluation metrics to estimate the quality of}
% \sys's
% \st{ clustering algorithm. Unlike CableMon}
% ~\cite{hu2020cablemon}
% \st{, it
% diagnoses the type of fault that causes an anomaly and can work with
% CableMon or other anomaly detection systems.}

% Processing (NLP) to parse the raw ticket text. have also attracted
% attentions of previous researches. Potharaju
% \ea~\cite{potharaju2013juggling} propose to leverage the raw ticket
% text for diagnosing network issues and recommend
% actions. LOTUS~\cite{venkataraman2018assessing} relies on Natural
% Language Processing (NLP) to parse the raw ticket text.
% CableMon~\cite{hu2020cablemon} uses tickets as hints to guide
% searching metric thresholds for detecting outages.


% \paragraph{Fault diagnosis in data center networks} 
% Narya's
% effectiveness is demonstrated by its deployment in
% Azure~\cite{copeland2015microsoft}.  


% \zzy{Delete this paragraph?} Narya~\cite{levy2020predictive} is a system that uses a reinforcement
% learning model and network telemetry data to predict host failures and
% suggest mitigation actions in datacenter networks, while \sys uses
% unsupervised learning for fault diagnosis in cable networks. 

\iffalse
\xy{We can remove this paragraph. Criteria for inclusion: related technology or same problem domain. I think it's safe to leave out IP-layer trouble shooting work.}
Both 007~\cite{arzani2018007} and Spidermon~\cite{wang2022closed}
employ active probing to collect network data for
troubleshooting. Among them, 007 uses path intersection to pinpoint
problematic links, and Spiderman uses a dependency graph to diagnose
root causes of network faults. Differently, \sys uses the existing
telemetry infrastructure in cable networks and unsupervised learning
for fault diagnosis.

Several proposals innovate network monitoring and troubleshooting
systems. Trumpet~\cite{moshref2016trumpet} uses a central controller
to install triggers at end systems for network-wide event
monitoring. Pathdump~\cite{tammana2016simplifying} and
SwitchPointer~\cite{tammana2018distributed} include extra information
in packet headers for network troubleshooting.  \sys is a
physical-layer fault diagnosis system and does not require changes in
network telemetry infrastructure. 
\fi

% Hauer~\etal~\cite{hauer2020meaningful} propose a met-
% ric measuring availability with their experience of Google’s
% service downtime. While it is the most relevant work in the
% literature focusing on downtime, i.e., missing data points in
% the context of this paper,
% 
% 
%  and ~\cite{iqbal2022characterizing} systematically measure the
% availability and latency in Amazon Web Services
% (AWS)~\cite{amazon2015amazon}.
% 
% 
% that has a global view of
% the network for fault
% diagnosis~\cite{,tammana2018distributed,}.
% 
% The
% central controllers can usually provide a global view to the network
% states but can also require significant deployment
% efforts. Moreover,~\cite{tammana2016simplifying,tammana2018distributed}
% also need to embed information into packet header, which makes the
% deployment even more convoluted.
% 
% 
% 
% 
% 
% 
% 
%   Besides relying on the measurement
% data, previous
% work~\cite{wang2022closed,arzani2018007,iqbal2022characterizing} has
% also employed active probing to collect data for
% troubleshooting. Among them,~\cite{wang2022closed} requires to build a
% dependency graph,~\cite{arzani2018007} traces packet trajectories,
% and~\cite{iqbal2022characterizing} systematically measure the
% availability and latency in Amazon Web Services
% (AWS)~\cite{amazon2015amazon}.  Comparing to the previous work, \name
% is built based on the PNM infrastructure that is already defined in
% DOCSIS and deployed in ISP's networks and does not need any additional
% deployment efforts. The PNM infrastructure is a passive monitoring
% system that does not introduce any probing packets.

% Log analysis: ~\cite{yu2011profiling}

% Fault Diagnosis and Prediction on Cloud: ~\cite{levy2020predictive}

% Availability on Cloud: ~\cite{iqbal2022characterizing}

% Active probing: ~\cite{wang2022closed,arzani2018007}

% Central controller: ~\cite{tammana2016simplifying,tammana2018distributed,moshref2016trumpet}

% Analyze missing data: ~\cite{hauer2020meaningful}

% \paragraph{Anomaly detection in Online Social Networks}

% detection fake account using clustering: ~\cite{cao2012aiding, cao2014uncovering}

% \paragraph{Anomaly detection in cable networks} Specifically for cable broadband networks, the Measuring Broadband
% America project~\cite{fcc2011} has been launched by the
% Federal Communications Commission since 2010.
% Padmanabhan \ea~\cite{padmanabhan2019residential} reveal the correlation between network outages and bad weather conditions.
% Researchers have designed frameworks and algorithms to detect
% networking issues based on data collected from real-world markets.



% However, unlike \name, its design only focuses on a
% single cable modem and cannot tell the correlation among multiple
% devices. Previous work~\cite{hu2022characterizing} has also deeply
% analyzed packet loss characteristics in cable networks. That effort is
% orthogonal to \name as packet loss is considered as one of the metrics
% indicating anomalies, but \name does not reason about the
% characteristics of each metric.
% 
% Our previous work: cablemon, physical layer loss



==> related_old.tex <==
\section{Related Work}


\xy{Cite this: https://www.microsoft.com/en-us/research/publication/towards-a-cost-vs-quality-sweet-spot-for-monitoring-networks/} \zzy{Done}

\xy{Cite this: https://www.microsoft.com/en-us/research/publication/007-democratically-finding-the-cause-of-packet-drops/} \zzy{Already cited ~\cite{arzani2018007}}

\xy{For this subsection, can you describe what methods each paper uses to detect anomaly or diagnose a fault? We need to compare methodology differences.} \zzy{Added more details.}

\paragraph{Anomaly detection in data center networks} Cloud services supported by data center networks are becoming popular with the emerging of the requirements of various service level objectives. One of the goals for a cloud service provider is to guarantee the overall system availability and meet the customers' demands. In literature, there is plenty of work aiming for troubleshooting anomalies in data center networks based on collected data reflecting network states. Yaseen \ea~\cite{yaseen2021towards} propose a framework efficiently collecting telemetry data without downgrading data quality. Narya~\cite{levy2020predictive} is designed based on reinforcement  learning models taking in network telemetry data to predict host failures and suggest mitigation actions. Narya's effectiveness is demonstrated by its deployment in Azure. % ~\cite{copeland2015microsoft}. 
Hauer \ea~\cite{hauer2020meaningful} propose a metric measuring availability with their experience of Google's service downtime. While it is the most relevant work in the literature focusing on downtime, \ie, missing data points in the context of this paper, \name also takes the value of non-missing data points into consideration and performs clustering based on their patterns. 
SNAP~\cite{yu2011profiling} collects TCP statistics and socket-level logs to pinpoint root causes by finding the correlations among multiple flows' statistics. \sys also leverages similarity for clustering but unlike SNAP, which can only produce a binary output as normal or abnormal, \sys can tell apart multiple maintenance or service issues simultaneously. 
A central controller can also be introduced for diagnosis systems~\cite{tammana2016simplifying,tammana2018distributed,moshref2016trumpet}. The central controllers can usually provide a global view to the network states but can also require significant deployment efforts. Moreover,~\cite{tammana2016simplifying,tammana2018distributed} also need to embed information into packet header, which makes the deployment even more convoluted.
Besides relying on the measurement data, previous work~\cite{wang2022closed,arzani2018007,iqbal2022characterizing} has also employed active probing to collect data for troubleshooting. Among them,~\cite{wang2022closed} requires to build a dependency graph,~\cite{arzani2018007} traces packet trajectories, and~\cite{iqbal2022characterizing} systematically measure the availability and latency in Amazon Web Services (AWS)~\cite{amazon2015amazon}.  Comparing to the previous work, \name is built based on the PNM infrastructure that is already defined in DOCSIS and deployed in ISP's networks and does not need any additional deployment efforts. The PNM infrastructure is a passive monitoring system that does not introduce any probing packets. 

% Log analysis: ~\cite{yu2011profiling}

% Fault Diagnosis and Prediction on Cloud: ~\cite{levy2020predictive}

% Availability on Cloud: ~\cite{iqbal2022characterizing}

% Active probing: ~\cite{wang2022closed,arzani2018007}

% Central controller: ~\cite{tammana2016simplifying,tammana2018distributed,moshref2016trumpet}

% Analyze missing data: ~\cite{hauer2020meaningful}

\paragraph{Anomaly detection in Online Social Networks} Another use case of clustering-based anomaly detection is fake account detection in Online Social Networks. Previous work~\cite{cao2012aiding, cao2014uncovering} reveals the effectiveness of applying clustering algorithms onto social networks to recognize accounts with abnormal behavior patterns as fake accounts. \name shares similar ideas for clustering with this previous work but also faces unique challenges for the \pnmdata coming from cable networks. For example, as a result of the unreliable transmission protocol, missing points caused by packet loss are common while the studies for Online Social Networks do not have this challenge.

% detection fake account using clustering: ~\cite{cao2012aiding, cao2014uncovering}

\paragraph{Anomaly detection in cable networks} Specifically for cable broadband networks, the Measuring Broadband
America project~\cite{fcc2011} has been launched by the
Federal Communications Commission since 2010.
Padmanabhan \ea~\cite{padmanabhan2019residential} reveal the correlation between network outages and bad weather conditions.
Researchers have designed frameworks and algorithms to detect networking issues based on data collected from real-world markets. CableMon~\cite{hu2020cablemon} applies simple threshold approach to detect anomalies. However, unlike \name, its design only focuses on a single cable modem and cannot tell the correlation among multiple devices. Previous work~\cite{hu2022characterizing} has also deeply analyzed packet loss characteristics in cable networks. That effort is orthogonal to \name as packet loss is considered as one of the metrics indicating anomalies, but \name does not reason about the characteristics of each metric.

% Our previous work: cablemon, physical layer loss

\paragraph{Clustering algorithms for anomaly detection} Previous researchers also introduce novel ideas for detecting anomalies on time series data~\cite{zhang2016taskinsight, li2021clustering}. Wu \ea~\cite{wu2016survey} classified the anomaly detection algorithms into five categories according to the detection criteria: based on statistical, clustering, deviation, distance and density. Ferreira \ea~\cite{ferreira2016time} propose to employ community detection for clustering of time series data. \name's clustering algorithm is similar to the proposed algorithm but has also been elaborately adjusted for the challenges raising by cable networks such as data alignment. 

% Time series clustering using community detection: ~\cite{ferreira2016time}

% using clustering to detect anomaly: ~\cite{zhang2016taskinsight, li2021clustering}

% a survey on anomaly detection on time series data ~\cite{wu2016survey}

\paragraph{Customer ticket analysis} Customer report tickets have also attracted attentions of previous researches. Potharaju \ea~\cite{potharaju2013juggling} propose to leverage the raw ticket text for diagnosing network issues and recommend actions. LOTUS~\cite{venkataraman2018assessing} relies on Natural
Language Processing (NLP) to parse the raw ticket text.
CableMon~\cite{hu2020cablemon} uses tickets as hints to guide searching metric thresholds for detecting outages.


==> results_analysis.tex <==
\subsection{Ticket Reporting Rate}
\label{sec:result_stats}
\jy{ready to read}
%In this subsection, we will introduce several interesting findings from the maintenance issues and service issues \sys detected. We assume all the detection results outputted by \sys are correct based on the evidence supported in~\S~\ref{sec:manual_label} and~\S~\ref{sec:ticketing_rate}. We will first show the geographical distribution of devices affected by the same maintenance. Then, we will show how many customers will report tickets when a maintenance issue happens. Last, we will show the difference in ticket statistics from service and maintenance issues \sys detect.

In this subsection, we will introduce several interesting findings from the maintenance issues and service issues \sys detected. We assume all the detection results outputted by \sys are correct based on the evidence supported in~\S~\ref{sec:manual_label}, ~\S~\ref{sec:ticketing_rate}, and ~\S~\ref{sec:ticket_characteristics}. We will first show how many customers will report tickets when a maintenance issue happens. Then, we will show the difference in ticket statistics from service and maintenance issues detected by \sys.

\if 0
\begin{figure}[t!]
\centering
    \includegraphics[width=.45\textwidth]{./figures/distance_ratio.eps}
    \caption{\small\textbf{The average distance ratio for the maintenance issues detected by each performance metric.}}
    \label{f:distance_density}
\end{figure}


\begin{figure}[t!]
\centering
    \includegraphics[width=.45\textwidth]{./figures/group_size.eps}
    \caption{\small\textbf{The group size ratio for the maintenance issues detected by each performance metric.}}
    \label{f:group_size}
\end{figure}


\textbf{Group Size and Geographical Distribution.} In Figure~\ref{f:tx_power_examples_map}, we show that the cable devices that share the same abnormal patterns on Tx power are close to each other. We are curious whether this phenomenon is common for all the maintenance issues on all performance metrics. Therefore, for each maintenance issue \sys detected, we calculate the average distance between all cable devices and the centroid of this maintenance issue. We obtain the centroid of each maintenance issue by calculating the mean of latitudes and longitudes among all the cable devices enrolled in this maintenance issue. Then, we calculate \emph{average distance ratio}, which means the average distance for a maintenance issue divided by the average distance for the entire fiber-optic node. A low average distance ratio represents that the devices affected by the same maintenance issue tend to aggregate in the same geographical location. 

Figure~\ref{f:distance_density} shows the CDF of the average distance ratio for the maintenance issues detected by each performance metric. We can observe that for the issues detected by SNR and missing, the average distance ratio is around 1 for most maintenance issues, indicating that the affected devices are scattered in different geographical areas. The issues detected by transmission power show a different trend. More than 20\% of the maintenance issues have an average distance ratio of less than 0.5, while more than 40\% of the maintenance issues' values are less than 0.75, which shows a consistent pattern shown in Figure~\ref{f:tx_power_examples_map}.

However, we notice that the average distance ratio cannot reflect the influence of the size of a maintenance issue. If a maintenance issue affects all the cable devices in the same fiber optic node, the average distance ratio should always be 1. Therefore, we define group size ratio, which uses the number of devices affected by a maintenance issue divided by the number of all the devices in the same fiber optic node, to show the characteristics of different performance metrics. Figure~\ref{f:group_size} shows the CDF of group size ratio for different performance metrics. The issues detected by missing and SNR also have a similar distribution, showing those maintenance issues have a higher probability of affecting most of the devices in the same fiber optic node than the maintenance issue detected by transmission power. 
\fi

\begin{figure}[t!]
\centering
    \includegraphics[width=.45\textwidth]{./figures/ticket_report_rate.eps}
    \caption{\small\textbf{The ticket report rate for the maintenance issues
detected by each performance metric.}}
    \label{f:ticket_report_rate}
\end{figure}


\textbf{How Many Customers Will Report Tickets?} When a network issue affects customer experience, a customer may report a ticket to complain about this issue. However, not all customers will report a ticket if a maintenance issue affects multiple customers. Besides, customers may not report the issue immediately when the issue happens. So in this part, we are curious about how many customers will report a ticket when a maintenance issue happens. In this study, we only consider the maintenance issue that received at least one maintenance ticket to mitigate the false positive in our detection results. We quantify the question by \emph{ticket report rate}, which means the percentage of customers that report tickets for a maintenance issue. Figure~\ref{f:ticket_report_rate} shows the CDF of ticket report rates. The result shows that, for more than 80\% of the maintenance issues (detected by any performance metric), 90\% of the customers will not report tickets.

\textbf{Service Tickets vs. Maintenance Tickets}\jy{Need to refine or remove this section}
Our ticket data is noisy. A service ticket may be labeled as a maintenance ticket and vice versa. To quantify the noise in our ticket data, we compare how many tickets captured by the maintenance issues are service tickets and how service issues capture maintenance tickets. Our ticket data contains 56.07\% service tickets and 43.96\% maintenance tickets. Among the tickets captured by service issues, there are 82.57\% service tickets and 17.43\% maintenance tickets, while our maintenance issues captured 64.34\% of maintenance tickets and 35.66\% of service tickets. This result shows a significant statistical difference compared to the distribution among all tickets. 

Besides, we also check how many maintenance tickets captured by the same maintenance issues are assigned to two or more primary tickets. From the maintenance issue that at least captured 1 part of the primary ticket, we observed that 27.15\% of them captured the tickets with two or more primary tickets.

==> results_external_criteria.tex <==
% \subsection{Manual-Label-Based Evaluation}
% \label{sec:manual_label}
% 
\if 0
\begin{table}[t!]
% \scriptsize
% \small
\centering
\begin{tabular}{c c c c c}
% \toprule
                    & \sys & DBSCAN & \makecell[c]{Single \\ Linkage}  & \makecell[c]{Complete \\ Linkage} \\ \toprule
% Purity              & 0.96  & 0.88 & 0.88 & 0.94 \\ \midrule
RI                  & 0.91  & 0.84 & 0.83 & 0.83 \\ \midrule
ARI                 & 0.83  & 0.65 & 0.64 & 0.66 \\ % \bottomrule
\end{tabular}
\caption{\small\textbf{Rand Index and Adjusted Rand Index for various clustering algorithms.}\label{tab:manual_label_result}}
\end{table}
\fi

We run \sys on the \pnmdata we label and compare \sys's diagnosis
results with our labeled results.  We also compare \sys's choice
of the clustering algorithm, the average-linkage clustering
algorithm, with three alternatives: DBSCAN, single-linkage, and
complete-linkage clustering
algorithm.  We choose two
widely-used metrics for evaluating each clustering algorithm: the Rand
Index (RI)~\cite{rand1971objective} and the Adjusted Rand Index
(ARI)~\cite{hubert1985comparing}.

We compute RI by comparing the partitions produced by a clustering
algorithm with the ground truth partition.  If two devices are in the
same cluster in both partitions, we count it as a true positive
($TP$).  Conversely, if two devices are in the same subset in the
partition produced by a clustering algorithm, but they are in
different subsets in the ground truth partition, we count it as a
false positive ($FP$). True negatives ($TN$) and false negatives
($FN$) are defined accordingly. The Rand Index computes the fraction
of true positives and negatives divided by the total pairs of devices:
$\frac{TP+TN}{TP+TN+FP+FN}$. Its maximum value is 1. The higher the
RI, the better a clustering result.  ARI adjusts for the random
chances that a clustering algorithm groups two devices in the same
cluster by deducting the expected RI ($\mathbb{E}(RI)$) of a random
partition: $\frac{RI-\mathbb{E}(RI)}{1-\mathbb{E}(RI)}$.

% If the number of devices in each cluster is imbalanced, for instance,
% the partition only consists of a large group of devices affected by a
% maintenance issue and a small group of devices not affected by the
% issue, the Rand Index may still be high even if a clustering algorithm
% partitions all devices in the smaller cluster into the larger
% cluster. The Adjusted Rand Index introduces a normalization mechanism
% to alleviate this problem. 

Table~\ref{tab:manual_label_result} shows the comparison results. \sys
achieves an RI of 0.91 and an ARI of 0.83, respectively. It
outperforms other clustering algorithms.

% This design does not affect \sys's
% effectiveness, as it can still distinguish maintenance issues from
% service issues. \zzy{This is not \sys's design, but an evaluation design, so I % don't think it could ever affect \sys's effectiveness because they are irrelevant.}

% 
% \begin{itemize}
% \item
% %    \emph{Purity} is calculated by summing up the number of elements
% %    (\ie, devices in our case) for the majority class in each cluster
% %    (\ie, maintenance or service issue in our case), divided by the
% %    total number of elements.
% 
%    Formally speaking, $\mathrm{purity}(\Omega, \mathbb{C}) = \frac{1}{N}\sum\limits_{k}\max\limits_{j}|\omega_k\cap c_j|$, where $\Omega = \{\omega_1, \omega_2, ..., \omega_K\}$ is the set of clusters and $\mathbb{C} = \{c_1, c_2, ..., c_J\}$ is the set of classes. 
% 
%  \item
%    \emph{Rand Index (RI)}~\cite{rand1971objective} is a measure of the similarity between two  clusters. Let $a$ denote the number of pairs of elements that are in the same subset of both clusterings, and $b$ denote the number of pairs of elements that are in different subsets of both clusterings, then $\textrm{RI} = \frac{a+b}{\tbinom{n}{2}}$, where $n$ is the number of elements.
% 
%  \item
%    \emph{Adjusted Rand Index (ARI)} is a commonly used evaluation metrics for unsupervised clustering algorithms built upon RI. Intuitively, ARI measures how similar two cluster results are. Formally, $\textrm{ARI} = \frac{\textrm{RI - expected(RI)}}{\textrm{max(RI) - expected(RI)}}$. 
% % , where RI is defined as the accuracy on pairs of points. 
% % show the performance and compare our method to other methods: Table 1\\
% 
% \end{itemize}

% The details for each metric can be found in Appendix~\ref{appendix:clutering_metrics}. Intuitively, they are measuring how similar the clustering result is to an ideal partition on the dataset.
% 
% The result shows that \sys outperforms other algorithms in all metrics, and all other algorithms show similar performances. This reveals that algorithm based on density, such as DBSCAN, are not good options for clustering network telemetry data because  missing data points are inevitable in practice. And such missing points introduce varied-length vectors for each sample and thus they cannot be mapped into a space with a fixed dimension for estimating density. As for hierarchical clustering, there are three ways to define the similarity for clusters: single-linkage, complete-linkage and group average. \zzy{Which one are we using for comparison?} The first 2 variants are sensitive to noises and hierarchical clustering with group average is less efficient than \sys. 
% \jy{need to rewrite this paragraph}




==> similiarity.tex <==
\subsection{Similarity Comparison}
\label{sec:similarity}



In order to compare the similarity of the time series data between two
different devices, we need to find good similarity metrics. However,
since our data contains different types of performance metrics, we may
use different similarity metrics for different types of
metrics. Specifically, we divide our performance metrics into three
categories: instantaneous metrics, accumulated metrics, and missing.

\textbf{Instantaneous Metrics}: The instantaneous metrics indicate the status of a device at the time we collected these metrics, including TX power, RX power, and SNR in our data. Figure~\ref{f:pattern_sample_new} shows an example of TX power, one of the instantaneous metrics in our data. We can observe that for the instantaneous metrics, the devices affected by the same anomaly have a similar shape. Therefore, we select Pearson correlation coefficient~\cite{benesty2009pearson} as the similarity/distance metric for the instantaneous metrics. There are several reasons for us to select this metric. Firstly, the RF impairments will affect multiple devices at the same time, so we will have no time distortion. Therefore, we should apply lock-step measures, which prevent us from using elastic measures such as DTW. Secondly, although instantaneous metrics collected from abnormal devices have a similar shape, they have different scales. Therefore, some classic distance metrics such as Euclidean distance cannot work well. Thirdly, since we have missing data, we need to calculate the different pair-wise distances with different lengths of input vectors. All the above challenges can be solved by the Pearson correlation coefficient, which measures the linear correlation between two input vectors. 

\if 0
\textbf{Accumulated Metrics}: Accumulated metrics mean the change of accumulated counter between the current and its previous data collection point, representing the condition of devices during the last 4 hours (our data collection interval). In our data, the accumulated metrics include uncorrectable codewords, correctable codewords and unerrored codewords. In this work, we only use the codeword error rate, which is calculated using the number of uncorrectable codewords divide by the sum of all types of codewords. However, different from the instantaneous metrics that are only influenced by the instantaneous status of devices, codeword error rate can be affected by customer behavior during a long time period. If a device sends very few codewords during the last 4 hours, or status of the devices keeps changing between good and bad but the devices only send a huge amount of data when the status of devices are bad, then their codeword error rate will be significantly different from the devices that constantly send the data. Due to these reasons, the shape of different vectors could vary, which prevent us from applying the Pearson correlation coefficient. To solove this challenging, we first get rid of the data points with too few codewords sent during the last 4 hours, and label these data points as missing, so that we can obtain the same $V_{a'}$ using the method described in Section~\ref{sec:align}. Then, we generated $V_a$ by $V_a = \{1 \ $ if $ v_t $ > threshold else $0 \ | v_t\in V_{a'}\}$. For each device in our dataset, we will obtain a vector with elements 0 and 1. 1 means abnormal and 0 means normal. We use the algorithm described in CableMon~\cite{hu2020cablemon} to determine the value of threshold. \zzy{Because the submission is double-blind, it might be better to state that we get the approval and implementation of the authors of CableMon, or sth like that.}\jy{I think we should mention it in previous sections} After obtaining the vector of each device, we apply the 
Normalized Hamming distance as our similarity/distance metric, which
means the Hamming distance divided by the length of the input
vectors. Hamming distance is the most popular metric to calculate the
distance between binary
strings~\cite{tammana2018distributed}. However, due to the missing
data we have , we need to calculate the different pair-wise distances
with different lengths of input vectors. So we use Normalized Hamming
distance to avoid this issue.
\fi 

\textbf{Missing}: Missing is an important metric since it indicates the availability of the cable broadband network. Many factors can cause missing, e.g., the SNMP request or response packet was dropped due to packet loss, customers turn off the power of their devices, or the device is broken so that it cannot send or receive any data. In order to use the missing as the availability indicator, we only focus on the missing data shown in all of the 3 channels at the same time. When we collect the data, we will collect the PNM data from all the 3 upstream channels at the same time. If there is only 1 or 2 channels missing, we will not consider this missing indicates availability issue. \zzy{May need to state the reason briefly, eg. the device has LB mechanisms.} However, missing is not included in our raw dataset, Therefore, we use the algorithm described in Section~\ref{sec:align} to infer the place of the missing in our data. For device $a$ and device $b$, $|T_a| \ = \ |T_b|$, if we start and finish to collect the data from both of these devices at the same time. Therefore, we can generate the missing vector $V_a = \{1$ if missing at $t_i$ else $0 \ | t_i \in T_a\}$ and $V_b$ use the same method. Then, $|V_a|$ should be the same as $|V_b|$. For each device in our dataset, we will obtain a vector with elements 0 and 1. 1 means we have data at this timestamp, and 0 means missing. After obtaining the vector of each device, we apply the Normalized Hamming distance as our similarity/distance metric, which means the Hamming distance divided by the length of the input vectors. Hamming distance is the most popular metric to calculate the distance between binary strings~\cite{tammana2018distributed}. However, due to the missing data we have , we need to calculate the different pair-wise distances with different lengths of input vectors. So we use Normalized Hamming distance to avoid this issue.

%\subsection{Clustering the Modems with Incomparable Patterns}\label{sec:cluster}


==> ticket_characteristics.tex <==
\subsection{Ticket Characteristics}
\label{sec:ticket_characteristics}
\jy{ready to read}
Besides the normalized ticking rate, in this section, we use the ticket characteristics as evidence to show that \sys can effectively distinguish service issues from maintenance issues using \pnmdata. We use the ticket waiting time and ticketing interval as evaluation metrics in this section. We will define them on first use. 

\if 0
\paragraph{Report Wait Time.} In ~\cite{hu2020cablemon}, the authors use the metric \emph{report wait time} to support the validity of CableMon. The report wait time is how long it takes from the start of a network anomaly to the time the first ticket is reported. Short reporting wait times mean serious network problems. \sys separates maintenance issues from service issues, and we assume that maintenance issues will have shorter wait times for ticket reports compared to service issues. To test this hypothesis, we plot the reporting wait time CDF for maintenance and service issues detected by \sys, as shown in ~\ref{f:report_waiting_time}. There was no difference between maintenance issues and service issues when reporting wait times were shorter. It shows a significant difference when the ticket reporting time is long, indicating the maintenance issues \sys detected are statistically significant to be a true maintenance issue. 
\fi


\paragraph{Ticket Waiting Time}

\begin{figure}[h]
\centering
    \includegraphics[width=.45\textwidth]{./figures/report_waiting_time_type.eps}
    \caption{\small\textbf{The ticket waiting time for maintenance and service issues detected by \sys.}} % \jy{redraw the figure}
    \label{f:report_waiting_time}
\end{figure}

The first ticket metric we use for evaluation is the ticket waiting
time. We define it as the first trouble ticket arrival time after an
anomaly event occurs. \zzy{What if there're no tickets coming?} If we assume that each user's ticket waiting
time for an anomaly is randomly distributed, and a maintenance issue
affects more subscribers than a service issue, then the ticket waiting
time for a maintenance issue should be shorter than that for a service
issue. If \sys correctly separates the two issues, we should observe
the differences in the ticket waiting time distributions between a
maintenance issue and a service issue. 

Figure~\ref{f:report_waiting_time} shows the ticket waiting time
distributions for anomaly events diagnosed as maintenance issues and
service issues by \sys, respectively. Note that we do not differentiate the
first arrival ticket's type for an event, as it may be mis-labeled by
an operator. We observe that when the ticket waiting time exceeds a
few hours, there is a significant difference between the ticket
waiting time distribution for maintenance issues and that for service
issues. For example, for more than 50\% of the maintenance issues
diagnosed by \sys, the first ticket arrives within 24 hours. In
contrast, only for less than 23\% of the service issues diagnosed by
\sys, the first ticket arrives within 24 hours. This difference again
suggests that \sys is able to separate maintenance issues from service
issues effectively. Interestingly, we note that when the ticket waiting time is
short, the ticket waiting time distributions for maintenance and
service issues overlap. We hypothesize that these tickets are impacted
by severe issues so that any subscriber impacted by one of these
issues reports immediately.

\begin{figure}[h]
\centering
    \includegraphics[width=.45\textwidth]{./figures/ticket_time_interval.eps}
    \caption{\small\textbf{The cumulative distributions of ticketing
        intervals for maintenance issues, service issues, and the
        entire data collection period.}} % \jy{redraw the figure}
    \label{f:ticket_time_interval}
\end{figure}

\paragraph{Ticketing Interval}
The second ticket metric we employ to evaluate \sys is the ticketing
interval. We define it as the time interval between two adjacent
tickets in the same \FN. 
We measure the ticketing interval for maintenance and service
issues, respectively. Based on \sys's diagnosis results, we divide
each device's data collection period as normal, a maintenance issue,
or a service issue. To measure a ticketing interval for maintenance
issues, we measure the time interval between two adjacent tickets that
occur in any device's maintenance period. Correspondingly, we measure
a ticketing interval for service issues. Because a maintenance issue
impacts more users than a service issue, more tickets will arrive
during a maintenance issue. In contrast, on average, one service
ticket should resolve one service issue. \zzy{Why cannot a single user reports multiple tickets for a service issue? I think only mentioning more affected users is sufficient. Or at least replace "on average" to "usually"?} Therefore, the ticketing
interval distribution for service issues captures the time interval
distribution between the occurrences of service issues. However, part
of the ticketing interval distribution for maintenance issues reflects
the synchronized ticket arrivals from multiple subscribers during a
maintenance event, while part of it reflects the time interval
distribution between the occurrences of maintenance issues.


Figure~\ref{f:ticket_time_interval} shows the cumulative distributions
of the ticketing interval for service issues, maintenance issues, and
the entire time collection period, respectively. We observe there are
significant differences between the ticket interval distributions for 
service issues and maintenance issues. For example, more than 60\% of
the ticketing intervals for maintenance issues are shorter than one
day; while only less than 14\% of the ticketing intervals for
service issues are shorter than one day. We note that when the
ticketing intervals are large ($>$ 10 days), the ticketing interval
distribution for maintenance tickets falls below the general ticketing
interval. We hypothesize that the ticketing intervals in this range
reflect the intervals between the occurrences of maintenance issues,
not the ticketing intervals within the same maintenance issues.


\paragraph{Network Issue Existing Time}

\begin{figure}[h]
\centering
    \includegraphics[width=.45\textwidth]{./figures/network_issue_existing_time.eps}
    \caption{\small\textbf{The cumulative distributions of existing time for maintenance issues and service issues}%\jy{redraw the figure}
    }
    \label{f:network_issue_existing_time}
\end{figure}

\jy{TODO}

 
% \textbf{Report Time Interval.} If multiple tickets are reported for the same maintenance issue, the reporting time interval between these should be small. Therefore, a short report time interval distribution will support the effectiveness of \sys. For all the tickets captured by the service issues and maintenance issues, \sys detected, we first group them by \FNs, then calculate the report time interval between any two adjacent tickets. Figure~\ref{f:ticket_time_interval} shows the CDF of the report time interval for tickets captured by service issues and maintenance issues. The maintenance issues \sys detected show a shorter report time interval.

% However, if one type of issue captures more tickets compared to the other type, theoretically it should have a shorter report time interval since the tickets are denser. The maintenance issues \sys reported capture nearly 4000 tickets, but the service issues only cover nearly 1000 tickets. It is possible that this distribution gap is caused by the density of tickets. In order to mitigate concern, we also show the report time interval distribution using all the tickets in our data, which contains more than 17000 tickets. The report time interval distribution of the tickets captured by maintenance issues still shows a shorter interval distribution, which indicates the maintenance issued \sys detected are statistically significant to be a real maintenance issue. We also observe that there is an intersection (10 days) between the tickets captured by maintenance issues and all tickets. We mark it as the time interval between two different maintenance issues that happened in the same fiber optic node.


\if 0
We noticed that the SNR provides a higher normalized maintenance ticketing rate. Firstly, compared to the transmission power, SNR is a direct metric to show the Quality of Service. If the SNR of a channel is lower, this channel will suffer a high packet loss rate~\cite{hu2022characterizing}, and affect customer experience. However, when we detect maintenance issues with transmission power, although it indicates the network is not working properly, it may not affect the customer experience. Cable devices will use a \emph{ranging process}~\cite{cablelabs2016docsis3} to adjust transmission power and other metrics, in order to compensate for the noise and impairments inside the channel. If it can compensate for the noise by increasing the transmission power, then the customers will not be affected by this issue, which prevents them from reporting more tickets. On the other hand, missing could be affected by many factors, e.g., an outage in the data collection server, or scheduled maintenance. If we can separate network issue related missing from other types of missing, we believe we will achieve a higher normalized maintenance ticketing rate in the future.
\fi

==> ticketing_rate.tex <==
\subsection{Normalized Ticketing Rates}
\label{sec:ticketing_rate}

To scale our evaluation beyond the manually labeled dataset, we
develop metrics based on customer tickets.  We split the 14-month
\pnmdata we have into two sets: an 11-month training set and a 3-month
test set. We use the training set to determine the values of \sys's
hyper-parameters (\S~\ref{sec:parameters}) and the test set to
evaluate the \sys's performance.

We define a normalized ticketing rate as a metric to evaluate \sys's
fault diagnosis accuracy.  Recall that in Eq~\ref{eq:rt_m} and
Eq~\ref{eq:rt_s}, we define two ticketing-rate variables
$R_{m,M}$ and $R_{m,S}$ as the number of maintenance
tickets averaged over the total length of data collection periods \sys
diagnoses as experiencing a maintenance and a service issue,
respectively. We can define ticketing rate variables $R_{s,M}$
and $R_{s, S}$ correspondingly where $s$ stands for service
tickets.

Because an ISP's fault diagnosis is inaccurate, we assume for each
type of ticket, there exists random errors. To discount those errors,
we define a baseline ticketing rate $R_{t}$ as the number of tickets
of type $t$ ($t$ is either maintenance or service) averaged over all
devices in a fiber optical node and the entire data collection period.

A normalized ticketing rate $\overline{R_{t,E}}$ of a ticket
type $t$ and a diagnosis type $E$, where $E$ is either a
maintenance issue or a service issue, is defined as
$\frac{R_{t,E}}{R_{t}}$. It puts a ticketing rate
$R_{t,E}$ into perspective. If we assume that an ISP receives a
much higher frequency of customer calls during a true maintenance or
service issue, then if a fault diagnosis system can accurately
diagnose a maintenance or service issue, we will observe a high
normalized ticketing rate for both maintenance and service issues. In
contrast, if a system cannot effectively identify maintenance or
service issues, we would observe a normalized ticketing rate close to
1.

% we expect that If a normalized ticketing rate is close to 1, it
% indicates that the diagnosis system
% 
% where $t$ denotes the type of a ticket (maintenance $m$ or service
% $s$) and $E$ denotes the type of a diagnosis (maintenance
% $M$ or service $S$).  A normalized ticketing rate
% $\overline{R_{t,E}}$ is defined as a ticketing rate normalized
% by the ticketing rate of the same ticket type ($R_{t}$) over the
% entire span of a dataset's data collection period:
%  Intuitively, the ticketing rate $R_{t}$
% models a random error in the customer ticketing and operator ticket
% classification process. If \sys obtains a high normalized ticketing
% rate for the diagnosed maintenance issues and service issues
% respectively, it is a strong indicator that its diagnosis is accurate.

The official PNM document from CableLabs~\cite{cablelabs2016docsis3}
describes a clustering algorithm that uses each \pnmdata point's
pre-equalization coefficients as a feature vector for clustering
devices impacted by the same linear RF distortions. As a comparison,
we implement this algorithm and set its clustering similarity
threshold in the same way as we tune those thresholds for \sys's
features, and compare the normalized ticketing rates defined in 

% \begin{table}[h]
% \scriptsize
% \centering
% \begin{tabular}{c c c c c}
% %\toprule
%          & \multicolumn{2}{c}{Maintenance Issues} & \multicolumn{2}{c}{Service Issues} \\\cmidrule{2-5}
%          & \makecell[c]{Maintenance \\ Tickets}  & \makecell[c]{Service \\ Tickets} & \makecell[c]{Service \\ Tickets}  & \makecell[c]{Maintenance \\ Tickets}\\ \midrule
% SNR         &  7.12     & 3.30  & 7.33 & 6.79        \\ \midrule
% Txpower     &  3.10     & 2.02  & 3.83 & 1.96        \\ \midrule
% Missing     &  6.86     & 2.67  & 13.00 & 2.63          \\ 
% \midrule
% Combined    &  4.28     & 2.40  & 8.01 & 2.02         \\ \midrule
% \makecell[c]{Pre-equalization \\ Coefficients} & 1.52 & 1.37 & 1.36 & 1.31
% % \bottomrule
% \end{tabular}
% \caption{\textbf{The values of different types of
%     normalized ticketing rates based on 
%     \sys's diagnosis result in \reactive.\jy{TODO: add ticket density for normal groups as well}\label{tab:our_ticket_density}}}
% \end{table}

% \begin{figure}[t!]
% \centering
%     \includegraphics[width=.7\textwidth]{./figures/our_ticket_density.eps}
%     \caption{\small\textbf{The normalized ticketing rates for various
%         combinations of 
%         ticket type and diagnosis result, where $m$ denotes
%         maintenance tickets, $s$: service tickets, $M$:
%         \sys-diagnosed maintenance issues, and $S$:
%         \sys-diagnosed service issues.}
%  % \zzy{``MM'' denotes $\overline{R_{m,M}}$, ``SS'' denotes $\overline{R_{s,S}}$, ``MS'' denotes $\overline{R_{m,S}}$, and ``SM'' denotes $\overline{R_{s,M}}$.}
%         \label{f:our_ticket_density}}
% \end{figure}

% \begin{figure}[t!]
% \centering
%     \includegraphics[width=.7\textwidth]{./figures/network_issue_existing_time.eps}
%     \caption{\small\textbf{The cumulative distribution of how long a
%         maintenance (or service) issue lasts.}
%     }
%     \label{f:network_issue_existing_time}
% \end{figure}


      
% For events diagnosed as maintenance issues, \sys's
% normalized maintenance ticketing rate is much higher than the
% normalized service ticketing rate for all features individually and
% the combined result. For events diagnosed as service issues, \sys's
% normalized service ticketing rate is higher than the normalized
% maintenance ticketing rate for all features individually and the
% combined result, but the difference between them for the SNR feature
% is small.

\if 0
\begin{table}[h]
% \scriptsize
\centering
\begin{tabular}{c c c c c}
% \toprule
            & \sys & DBSCAN & \makecell[c]{Single \\ Linkage}  & \makecell[c]{Complete \\ Linkage} \\ \toprule
SNR         & 8.54          & 5.39  & 6.50  & 7.00        \\ \midrule
Txpower     & 4.16          & 2.21  & 2.61  & 3.26        \\ \midrule
Missing     & 3.76          & 3.34  & 3.79  & 3.62         \\ \midrule 
Combined    & 3.95          & 2.65  & 2.98  & 3.31         \\ % \bottomrule
\end{tabular}
\caption{\textbf{Normalized maintenance ticketing rate for maintenance issues detected by different algorithms in \reactive.}\label{tab:normalized_ticketing_rate}}
\end{table}

Table~\ref{tab:normalized_ticketing_rate} shows the normalized maintenance ticketing rate for the maintenance issues detected by each performance metric among \sys and other clustering algorithms. This result indicates whether the customer reports more tickets during the maintenance issues each algorithm detected. From this table, we can observe that \sys achieves the highest normalized maintenance ticketing rate among all the algorithms we compared. For the maintenance issues detected by missing, the performance of \sys, single-linkage and complete-linkage hierarchical clustering algorithm is similar since missing contains less noise compared to other metrics. \zzy{Does that imply \sys's advantage is mainly to overcome noise? Otherwise why is the performance similar because of less noise?} 

We also compared the other three types of ticketing rates between \sys and
other clustering algorithms. Due to the space limit, we present the
results in Appendix~\ref{appendix:tables}. The results show that \sys consistently
outperforms other clustering algorithms.
\fi

% \subsubsection{\REACTIVE}
% 
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[h]
% \centering
% \begin{tabular}{cccc}
% % \cline{3-4}
% &             & \multicolumn{2}{c}{Ticket Label}          \\ \cline{3-4} 
% &             & M & S \\ \cline{2-4} 
% \multicolumn{1}{c}{\multirow{2}{*}{\makecell[c]{\sys's \\ Diagnosis}}} & M & 2147 ($TP$)       & 1062 ($FP$)    \\ \cline{2-4} 
% \multicolumn{1}{l}{}                                                                        & S     & 175 ($FN$)        & 1168 ($TN$)    \\ % \hline
% \end{tabular}
% \caption{\textbf{Confusion Matrix for Ticket Type. ``M'' denotes ``Maintenance'' and ``S'' denotes ``Service''.}\label{tab:confusion_matrix}}
% \end{table}


\input{op-knowledge.tex}
% TP: 362; TN: 293; FN: 35; FP: 260
% total tickets: 950



==> todo.tex <==
06/16/2023
Output features we used to determine anomaly to Wade

-- Ask Wade for a short description of the field test

Test 6h missing gap

-- Jiyao: test a little

Prepare presentation

-- Wait

Tobia's result?

-- Reach out to him

05/04/2023:
change table 2 mark
customer trouble tickets -> customer tickets
change $s$ to $s_f$
duplicate -> duplicated
change figure 23 from cross star to square and circle

05/03/2023:
time waiting time -> time reporting delay
check figure 7's data - Done
figure 8 -> draw ISP's label, and only use test data - Question
figure 6 -> change label 
show training set results for figure 6, 7, 8, and table 2


05/02/2023:
redraw figure 8 and 9, 10 use test data
get rid of table 2 and table 3
check whether the subsection is so big
check the formula of ai and ari
go through the section 6
cut white edge
figures 7 -> 1 line

05/01/2023:
TODO:
underline -> italics - Done
figure 2 -> Cut white edge to save space - Done
figure 3 -> Using a transparent image/Abnormaliry -> Fault/normal group -> healthy/>=5 -> C_{thr} (also add it to the parameter setting) - Done
no map for figure2 -  Done
figure 5 -> space  - Done
table3 -> percentage
table2->graph - Done
change the order of 6.4 and 6.5
get rid of section 7 for now
finish implementation 
xy: check whether we mention that a cluster is anomalous if any modem is considered anomalous

04/28/2023:
update the proactive evaluation results 
bring the implementation section back
change the point type for figure 2
redraw figure 6
add grid to figure 4567
change "Clustering Algorithm used by TelApart" in appendix
Ticket Report Rate --> Percentage of Customers Reporting a Ticket
notations should be consistent across main tex and appedix -> Done


09/16/2022
Writing Tasks:
1. Provide the relationship between SNR/Codewords and Tx/Rx power (Due: 09/14) - Working
2. Remove the efficiency part in our draft (Due: 09/14) - Done
3. Rewrite the infer missing part, and add more details on how we select this threshold using the clustering algorithm (Due: 09/21) - Working
4. Show more details on the design choice we select. Separate two different categories: not working/performance bad (Due: 09/28) - Working
5. Reorganize the struct of the paper, pay more attention to the evaluation part, and show the results instead of focusing on the methodology part (Due: 10/05)
6. Rewrite how to use Cablemon on this clustering work. (Due: 10/05)

Experiment Tasks:
1. Provide more data analysis on ticket and dataset description (Due: 09/14) - Working
2. Provide more data analysis on performance metrics and missing, and mention how this would help us diagnose and group modems with the same issue (Due: 09/21) - Working
3. Do more data analysis on missing, showing how it will reflect customer experience and what will affect missing. (Due: 09/28) - Working
4. Provide more analysis on user behavior/clustering characteristics (Due: 10/05)
5. Provide a comparison of our algorithm and other algorithms (not sure what to compare for now. Maybe mention frequency response clustering and show it does not work by word?)

Related work:
Robust System Instance Clustering for Large-Scale Web Services

04/20/2022

Future work:

* 7 days invocation
* integrate diagnosis vs. anomaly detection

04/19/2022
why we do not use kmeans
ndex [Hubert and Arabie
* Figure 8 & 9 can have service issues too, so as to illustrate the differences?


04/18/2022
change the figure from modem to device
show the metrics we are using
pnm data or telemetry data?


// 1) move pseudo code to appendix
2) try to fix the missing refs
3) complete evalu
4) add a limitation function
5) add some DTW discussion back
// 6) modem -> device
7) figure 5’s examples now have the same vector length
we need to show after insert missing, the vector length may still be different.


04/14/2022
t_l t_r -> t1, t2 - Done
change alignment figure - Done
write clustering section
check adjusted clustering results - Running

ticket reporting time for different metrics
count how many tickets can be detected by different metrics

04/13/2022
add the missing comparison for different clustering algorithms - Running

04/12/2022
draw map graph, and add service issue in our example draft - 04/12/2022 - Done


check how the txpower will be adjusted - 04/12/2022 - Done    https://www.ccexpert.us/telecommunications/power-ranging.html

snr/txpower/rxpower vs snr/txpower/rxpower - 04/12/2022 - Done

add the second reason that the community detect ions work better than other algorithms - Done

show the comparison to the adjusted algorithm for the hierarchical clustering - 04/12/2022 - Running



04/11/2022:

label z1 z2 z3 - Done
check qiang's ccs paper - Done



1. add missing evaluation Due: 04/11/2022 - Pending

2. show how many dispatches are wrong Due: 04/11/2022 - Done

two directions:
1. Not belong to the maintenance issue, but labelled as part of primary tickets: 7.0\%

2. More than 1 primary ticket observed in the maintenance issue we detected: 13.9\%



3. change table3 to other data format to show the comparison between service and maintenance issue we detected Due: 04/11/2022 - Done

For maintenance issue we detected: 47.6\% service tickets, 52.4\% part of primary tickets

For service issue we detected: 77.6\% service tickets, 22.4\% part of primary tickets

4. show DBScan and hierarchical comparison on ticket report time interval analysis Due: 04/11/2022 -  Done

5. find use cases in lessons.tex Due: 04/11/2022 - DCN uses SNMP, check spidermon

6. check we can add the comparison for X-means? -> use normalized data or change the distance metric Due: 04/12/2022 (de-prioritize) - do not need to do that

7. add run time and cost analysis Due: 04/12/2022 

8: find the explanation why the spectrum works better Due: 04/12/2022 

9. write done: why other linkage algorithm do not work.

10. In lessons.tex, discuss why spectrum-based algorithm works better?

8. add hierarchical comparison to the manually labeling results - Done

9. add combined results to ticket analysis - Done

todo 


